Plugin estimators for selective classification with out-of-distribution detection

Real-world classifiers can benefit from the option of abstaining from predicting on samples where they have low confidence. Such abstention is particularly useful on samples which are close to the learned decision boundary, or which are outliers with respect to the training sample. These settings have been the subject of extensive but disjoint study in the selective classification (SC) and out-of-distribution (OOD) detection literature. Recent work on selective classification with OOD detection (SCOD) has argued for the unified study of these problems; however, the formal underpinnings of this problem are still nascent, and existing techniques are heuristic in nature. In this paper, we propose new plugin estimators for SCOD that are theoretically grounded, effective, and generalise existing approaches from the SC and OOD detection literature. In the course of our analysis, we formally explicate how na\"{i}ve use of existing SC and OOD detection baselines may be inadequate for SCOD. We empirically demonstrate that our approaches yields competitive SC and OOD detection performance compared to baselines from both literatures.

==> chow_suboptimal.tex <==
% {We now show that the L2R and OOD problems share a common baseline.
% While this points at a connection between the problems, we show that this baseline may \emph{fail} for some important special cases of OOD detection.}

{We now show that the L2R and OOD problems share a common baseline;
however, 
this baseline may \emph{fail} for some important special cases of OOD detection.}


% We now take a closer look at the L2R and OOD detection problems, by establishing that the MSP baseline may \emph{fail} for the latter in some important special cases.

%
% \subsection{The maximum softmax probability baseline}
% \subsection{Common baseline: maximum softmax probability}
\subsection{Maximum softmax probability meets Chow's rule}

% While largely studied independently, both L2R and OOD detection share a simple yet effective baseline:
% given a scorer $f \colon \XCal \to \Real^L$ learned from training sample $S$ using a suitable loss function, 
% one computes softmax probability estimates $p_y( x ) \propto \exp( f_y( x ) )$.
% Samples with small maximum probability $\max_{y \in [L]} p_y( x )$
% are then adjudged to be worthy of abstention, or likely outliers.
% This baseline is 
% known as \emph{Chow's rule}~\citep{Chow:1970} in the L2R literature,
% % \todoakm{Nit: Chow's rule refers to the population rule. This is more like plugin Chow. I think Ni et al. just calls it confidence-based rejection. Hari: Chow seems a bit more specific than confidence-based rejection. In any case, we are now mainly using MSP to refer to this baseline.}
% and 
% the \emph{maximum softmax probability} (\emph{MSP}) score~\citep{Hendrycks:2017} in the OOD detection literature.
% % This baseline identifies samples for which the maximum softmax probability falls below a threshold, and either abstains on them (in the case of L2R) or declares them as OOD.

{
For inlier and outlier distributions $\Pr_{\rm in}, \Pr_{\rm out}$,
consider the L2R problem on $\Pr_{\rm in}$ and OOD detection on $\Pr_{\rm in}, \Pr_{\rm out}$.
We begin with an intriguing observation:
while developed in parallel strands of literature,
the \emph{confidence-based L2R baseline and maximum softmax probability OOD baseline are identical}.
Indeed, both baselines involve learning probability estimates 
$\hat{\Pr}_{\rm in}(y|x)$,
% $p_y( x )$, 
% \todoakm{Should we distinct $\Pr$ vs $\Pr_{\rm in}$?}
and using the score $\max_{y \in [L]} \hat{\Pr}_{\rm in}(y|x)$ to determine whether to reject a sample, or deem it OOD.

Does this imply that one may similarly employ other L2R methods for OOD detection, and vice-versa?
Conceptually,
L2R and OOD detection appear related:
both problems
% abstains from predicting on certain samples.
seek to identify certain ``abnormal'' samples.
However, 
% the reason for abstention is subtly different,
the notion of ``abnormal'' is subtly different,
as may be seen from their Bayes-optimal solutions~\eqref{eqn:chow},~\eqref{eqn:bayes-ood-detector}:
in L2R, 
% it is for samples where 
we identify samples where
% $\Pr_{\rm in}( y \mid x )$ is insufficiently peaked,
$\max_{y \in [L]} \Pr_{\rm in}( y \mid x )$ is small,
while in OOD detection,
% In the OOD detection problem, it is for 
we identify
samples where 
$\frac{\Pr_{\rm in}( x )}{\Pr_{\rm out}( x )}$ is small.
% the density ratio 
% $\frac{\Pr_{\rm out}( x )}{\Pr_{\rm in}( x )}$ 
% is large.

The absence of any consideration of $\Pr_{\rm out}( x )$ in L2R suggests 
the two problems may not be interchangeable after all.
% What, then, explains the popularity of the MSP baseline?
However, despite sharing a common baseline, {and the two problems generally acknowledged to be related \citep{yang2021generalized}}, there is surprisingly limited understanding of how precisely they relate to (and differ from) each other.
% Revisiting the formulations in \S\ref{sec:background},
% any such relation must involve further assumptions:
% the L2R problem involves a single distribution, while the OOD detection problem involves both an inlier and outlier distribution.

We now show that in two special cases of OOD detection (which impose specific assumptions on $\Pr_{\rm out}$),
the MSP baseline can be strongly \emph{sub-optimal} for OOD detection.}

% As a first step towards better relating the two problems, we show that the MSP baseline
% can in fact be suboptimal for a special case of OOD detection, known as \emph{open-set classification}~\citep{Scheirer:2013}, wherein the OOD samples come from an unseen class.
% \todoakm{Maybe MSP will be a more intuitive choice of name, rather than Chow's rule? Hari: changed here and elsewhere in this section}


%
\subsection{MSP may fail for uniform $\Pr_{\rm out}$}

As a warm-up, we first consider
\emph{density-based OOD detection}, 
where we assume $\XCal \subset \Real^D$ and $\Pr_{\rm out}$ is uniform.
Assuming
without loss of generality
that the volume of $\mathscr{X}$ is normalised to $1$,
the density ratio $\frac{\Pr_{\rm in}( x )}{\Pr_{\rm out}( x )} = {\Pr_{\rm in}( x )}$.
Thus,
from~\eqref{eqn:bayes-ood-detector},
the Bayes-optimal
OOD detector for 
\eqref{eqn:ood-detection-rate}
is simply
% \todoakm{Consistent notation}
$$ r^*( x ) = \indicator{\Pr_{\rm in}( x ) < \frac{\beta}{\alpha}}; $$
that is, we deem \emph{low-density} samples to be OOD.
By contrast, the MSP baseline deems samples where 
$\max_{y \in [L]} \Pr_{\rm in}( y \mid x ) < t$ to be OOD;
% \todoakm{Is it confusing that we now use $\Pr_{\rm in}$ rather than $\Pr$?}
that is, we deem \emph{low label-certainty} samples to be worthy of abstention.

% {Recall that the
% Bayes-optimal OOD detector for 
% \eqref{eqn:ood-detection-rate} 
% is
% $g^*( x ) = \indicator{r^*( x ) \geq \frac{\alpha}{\beta}}$
% for {density ratio} $r^*(x) = \frac{\Pr_{\rm out}( x )}{\Pr_{\rm in}( x )}$.
% % Suppose that $\Pr_{\rm out}$ is uniform over $\mathscr{X}$, 
% % and 

% Then,
% the optimal detector is simply $g^*( x ) = \indicator{\Pr_{\rm in}( x ) \leq \frac{\beta}{\alpha}}$;
% that is, we deem \emph{low-density} samples to be OOD.
% By contrast, recall that the Bayes-optimal L2R rule rejects samples where $\max_{y \in [L]} \Pr_{\rm in}( y \mid x ) < t$;
% \todoakm{$\Pr$ vs $\Pr_{\rm in}$}
% that is, we deem \emph{high label-uncertainty} samples to be worthy of abstention.

How well do these two rules align?
Observe that their decisions are based on fundamentally different quantities:
the marginal density $\Pr_{\rm in}( x )$,
and the class-probability $\Pr_{\rm in}( y \mid x )$.
Consequently, it is not hard to see that these rules might be at odds:
for a fixed joint distribution $\Pr_{\rm in}( x, y )$,
one may independently vary $\Pr_{\rm in}( x )$ and $\Pr_{\rm in}( y \mid x )$
such that low marginal {density} corresponds to \emph{high} {label-certainty}.
% Thus, MSP may make predictions that are completely at odds with the Bayes-optimal predictor;
Figure~\ref{fig:chow-fail-example} illustrates this in a simple one-dimensional setting.

The above makes precise 
observations that are implicit in prior work (e.g.,~\citet{Liu:2020b}),
% \proposal{and serves as an instructive warm-up}:
% \proposal{but may appear unsurprising}, 
% as it imposes a highly specific structure on $\Pr_{\rm out}$. 
{but may appear to be an artifact of the highly specific structure assumed on $\Pr_{\rm out}$.}
% as it imposes a highly specific structure on $\Pr_{\rm out}$. 
% that may not arise in practice.
% \proposal{it hints at a key distinction between L2R and OOD detection.}
% \todoakm{In light of previous work, can perhaps downplay claimed novelty/significance; say this is just a warm-up}
{However, we now show that 
even in OOD detection settings that appear tailored to MSP,
the latter can fail.}
% We now show that a similar result holds in a practically relevant setting.
% \todoakm{Restate: MSP seems more intuitive here}


%
% \subsection{Bayes-optimal open-set classification}
\subsection{MSP may fail for open-set classification}
\label{sec:chow-fail-open-set}

Our second setting is 
\emph{open-set classification}~\citep{Scheirer:2013}, 
wherein the OOD samples come from an unseen class.
% In \emph{open-set classification},
For example, suppose
the inlier distribution $\Pr_{\rm in}$ has support on all but one class $\YCal' = \YCal - \{ L \}$,
and the outlier distribution $\Pr_{\rm out}$ has support on the remaining class $L$.
We wish to reject samples from the unseen class at test time.
Formally, suppose the underlying distribution over samples from both the known and unseen classes is $\mathbb{P}^*( x, y ) = \pi^*( y ) \cdot \mathbb{P}^*( x \mid y )$.
The outlier distribution is $\Pr_{\rm out}( x ) = \Pr^*(x \mid y=L)$,
while
the training distribution is
% given by
\begin{align*}
    \PTr( x \mid y ) = \mathbb{P}^{*}( x \mid y )
    \quad
    \piTr( y ) = \frac{1( y \neq L )}{1 - \pi^*( L )} \cdot \pi^*( y ). 
    % \\
    %
    % \PTr( x \mid y ) &= \mathbb{P}^{*}( x \mid y ).
    %
\end{align*}
That is, the class-conditional distribution remains unchanged, but we rescale the label frequencies to only exclude the contribution of the unseen label.

% With this, we may derive the following.
% \todoakm{If needed we could omit this, since it is perhaps not of independent interest, and is just a means to proving Lemma 3.2, 3.3.}

% %
% \begin{lemma}
% \label{lemm:open-set-distribution}
% For the open-set setting with notional distribution $\Pr^*$ over all labels,
% the training distribution has
% \begin{align*}
%         %
%         \PTr( x, y ) &= \frac{1( y \neq L ) }{1 - \pi^*( L )} \cdot \mathbb{P}^*( x, y ) \\
%         %
%         \PTr( x ) &= \frac{\mathbb{P}^*( y \neq L \mid x )}{1 - \pi^*( L )} \cdot \mathbb{P}^*( x ) \\
%         %
%         \PTr( y \mid x ) &= \frac{1( y \neq L )}{\mathbb{P}^*( y \neq L \mid x )} \cdot \mathbb{P}^*( y \mid x ).
%     \end{align*}
% \end{lemma}

{
% \color{blue}
Now suppose our goal is to minimize the OOD detection error~\eqref{eqn:ood-detection-rate} for suitable $\alpha, \beta$.
% We have the following optimal detector.
The optimal detector is as follows.

%%% Commented by Hari -- move to appendix?
% Under this setting, the following optimises the OOD detection rate~\eqref{eqn:ood-detection-rate}.
% \begin{lemma}
% \label{lemm:bayes-open-set-ood}
% Under the open-set setting, the Bayes-optimal classifier for the OOD detection error $R_{\rm ood}( r ) \defEq \costin \cdot \Pr_{\rm in}( r( x ) = 1 ) + \costout \cdot \Pr_{\rm out}( r( x ) = 0 )$  takes the form:
% $$
% r^*(x) = 1
%     \,\iff\,
% \mathbb{P}^*( y = L \mid x ) \geq t_{\rm OPT},
% $$
% where $t_{\rm OPT} \defEq \frac{ \costin }{ \costin + \costout}$.
% \end{lemma}
%%%
\begin{lemma}
\label{lemm:bayes-open-set-rewrite}
 Under the open-set setting, the Bayes-optimal classifier for the OOD detection error 
%  $R_{\rm ood}( r ) \defEq \costin \cdot \Pr_{\rm in}( r( x ) = 1 ) + \costout \cdot \Pr_{\rm out}( r( x ) = 0 )$  
\eqref{eqn:ood-detection-rate}
takes the form:
% \resizebox{.99\linewidth}{!}{
    % \begin{minipage}{\linewidth}
        \begin{align*}
            r^*(x) = 1
            &\iff
            \mathbb{P}^*( y = L \mid x ) \geq \frac{ \costin }{ \costin + \costout} %\\
            % &
            \iff \max_{y' \neq L} \PTr( y' \mid x ) \geq \frac{\alpha + \beta}{\beta} \cdot \max_{y' \neq L} \mathbb{P}^*( y' \mid x).
        \end{align*}
%     \end{minipage}
% }
% This can be equivalently written as:
% The Bayes-optimal classifier for the open-set setting  in Lemma \ref{lemm:bayes-open-set-ood} can be equivalently written as:
% \todoakm{Perhaps we should write $t_{\rm opt}$, or just explicitly write it in terms of $\costin, \costout$. Hari: explicitly wrote the costs.}
% $$ \max_{y' \neq L} \PTr( y' \mid x ) \geq \frac{\max_{y' \neq L} \mathbb{P}^*( y' \mid x)}{1 - t}. $$
% $$ \max_{y' \neq L} \PTr( y' \mid x ) \geq \frac{\alpha + \beta}{\beta} \cdot \max_{y' \neq L} \mathbb{P}^*( y' \mid x). $$
\end{lemma}
}

%%% Commented by Hari -- move to appendix?
% The above simply formalises a intuitive strategy: 
% samples where the true class-probability $\Pr^*( y \mid x )$ places high confidence on the unseen label $L$ are likely to be OOD.
%%%


% \subsection{When does Chow's rule fail?}

Equipped with the Bayes-optimal classifier for the open-set setting,
let us
now consider the MSP baseline,
which deems a sample to be OOD iff $\max_{y' \neq L} \PTr( y' \mid x ) < t_{\rm MSP}$ for some $t_{\rm MSP} \in [ 0, 1 ]$.
% How well does this align with the Bayes-optimal classifier for the open-set setting (Lemma~\ref{lemm:bayes-open-set-ood}), which 
% deems a sample as OOD iff $\mathbb{P}^*( y = L \mid x ) \geq t$?
Importantly, here we consider the class-probability under the \emph{inlier} distribution $\PTr$.
% since by assumption we only have access to samples from this distribution.

%%% Commented by Hari
% How well does the MSP baseline align with the optimal rule from Lemma~\ref{lemm:bayes-open-set-rewrite}?
% Surprisingly, 
% \todoakm{Is it still surprising, given we already show this for the uniform case?}
% we show that %Chow's rule 
% MSP can make predictions that disagree with the optimal rule.
% \todoakm{Is this really opposite in a formal sense?}
%%% 

%%% Commented by Hari
% \begin{lemma}
% \label{lemm:bayes-open-set-rewrite}
% The Bayes-optimal classifier for the open-set setting  in Lemma \ref{lemm:bayes-open-set-ood} can be equivalently written as:
% % \todoakm{Perhaps we should write $t_{\rm opt}$, or just explicitly write it in terms of $\costin, \costout$. Hari: explicitly wrote the costs.}
% % $$ \max_{y' \neq L} \PTr( y' \mid x ) \geq \frac{\max_{y' \neq L} \mathbb{P}^*( y' \mid x)}{1 - t}. $$
% $$ \max_{y' \neq L} \PTr( y' \mid x ) \geq \frac{\alpha + \beta}{\beta} \cdot \max_{y' \neq L} \mathbb{P}^*( y' \mid x). $$
% \end{lemma}
%%%

% {\hari{Should we delete the equation below? It looks like just the original form of Chow's rule above is clear enough to point out the difference with the Bayes-optimal classifier}
% \color{red}
% To better understand this, observe that Chow's rule equally rejects iff:
% \begin{align*}
%     % \mathbb{P}_{\rm ood}( x ) &= \mathbb{P}^*( y = L \mid x ) \\
%     % \max_{y \neq L} \PTr( y \mid x ) < t &\iff \max_{y \neq L} \mathbb{P}^*( y \mid x ) < t \cdot ( 1 - \mathbb{P}^*( y = L \mid x ) ) \\
%     % &\iff \max_{y \neq L} \mathbb{P}^*( y \mid x ) < t - t \cdot \mathbb{P}^*( y = L \mid x ) \\
%     % &\iff t \cdot \mathbb{P}^*( y = L \mid x ) < t -\max_{y \neq L} \mathbb{P}^*( y \mid x ) \\
%     % &\iff 
%     \mathbb{P}^*( y = L \mid x ) < 1 - \frac{1}{t} \cdot \max_{y \neq L} \mathbb{P}^*( y \mid x ).
% \end{align*}
% }

%That is, we reject when the probability of the unseen class is
% That is, we reject when the maximum probability is
% \emph{lower} than some threshold.

On close inspection at both the classifiers, one can see that MSP can 
make predictions that 
starkly disagree with the optimal rule. More specifically, 
Lemma~\ref{lemm:bayes-open-set-rewrite} shows that the optimal decision is to reject when the maximum softmax probability (with respect to $\PTr$) is \emph{higher} than some (sample-dependent) threshold.
This is however the precise \emph{opposite} of the MSP baseline, which rejects when the maximum probability is
\emph{lower} than some threshold.
% \begin{align*}
% \max_{y' \neq L} \PTr( y' \mid x ) < t_{\rm MSP}.
% \end{align*}

What is the reason for this stark discrepancy?
% \todoakm{Maybe some of this can be pushed to Discussion}
Intuitively, the issue is that we would like to threshold the maximum of $\Pr^*( y \mid x )$, \emph{not} $\PTr( y \mid x )$;
however, these two distributions may not align,
as the latter includes a normalisation term that causes unexpected behaviour when we threshold.
% \todoakm{Change the markers}
We illustrate this with a concrete example (see also Figure~\ref{fig:chow-fail-example-open-set}). %

%
\textbf{Example (failure of MSP baseline)}.
Consider a setting where the class probabilities $\Pr^*( y' \mid x )$ are equal for all the known classes $y' \ne L$.
% Due to the normalization term, the inlier class probabilities then evaluates to become 
This implies that
$\PTr( y' \mid x ) = \frac{1}{L-1}, \forall y' \ne L$.
The Bayes-optimal classifier rejects a sample when 
% $\Pr^*( L \mid x ) > t_{\rm OPT}$.
$\Pr^*( L \mid x ) > \frac{\alpha}{\alpha + \beta}$.
% \todoakm{Since we reference the Bayes classifier here, I brought back the lemma we moved to the appendix, and merged it with Lem 3.1.}
On the other hand,
MSP rejects a sample 
iff the threshold 
$t_{\rm MSP} < \frac{1}{L-1}$.
% $t < \frac{1}{L-1}$.
Notice that rejection decision is \emph{independent} of the unknown class density $\Pr^*( L \mid x )$, 
and therefore will not agree with the Bayes-optimal classifier in general.
% Figure \ref{fig:chow-fail-example} illustrates this with examples of two open-set settings, where the inlier class probabilities are identical, but the unknown class probability varies across samples.

The following lemma formalizes the above observation.
% \todoakm{If needed maybe we can omit this; the point is clear enough at this stage I think. Hari: the only reason why a formal statement will be helpful is because we have two different thresholds, and we wish to say no matter what threshold we choose for MSP, one can always construct a distribution where it is at odds with the Bayes classifier.}
%
%
% {
% %\color{blue}
% The following lemma formalizes the above observation to show the existence of distributions where Chow's rule disagrees with the Bayes classifier.
\begin{lemma}
Suppose the MSP baseline is implemented as  $\max_{y \neq L} \PTr( y \mid x ) < t_{\rm MSP}$ for $t_{\rm MSP} \in (0, 1)$. 
Then for any choice of $t_{\rm MSP}$, there exists an underlying conditional-class distribution $\Pr^*(y \mid x)$ for which the Bayes-optimal classifier 
$\mathbb{P}^*( y = L \mid x ) \geq t$ disagrees with MSP $\forall t \in (0, 1)$.
\label{lem:chow-fail}
\end{lemma}

% \todoakm{Add an intuitive example where Chow's rule fails. Hari: added Fig \ref{fig:chow-fail-example}.}

% \todoakm{Add results on a synthetic problem where Chow's rule fails? Hari: good idea, will get to this soon after wrapping up current set of experiments}

% \todoakm{Given this is a common baseline that seems to work reasonably, can we identify settings where Chow's rule would work as expected? Hari: one setting where Chow will match the Bayes classifier is for all samples $x$, (i) one of the classes has a sufficiently $\Pr^*(y|x)$, and (ii) when it is the unseen class that receives the highest conditional probability, all other classes have near-equal and small probability, i.e.: $\Pr^*(y|x) \approx \frac{\beta}{\alpha + \beta} \cdot \frac{1}{L-1}$}

% %
% {
% \textbf{Example (illustration of failure of MSP baseline)}.
% Figure~\ref{fig:chow-fail-synthetic-example} presents a simple two-dimensional synthetic example where the maximum softmax probability fails.
% Here, while the Bayes-optimal score for the OOD samples tends to be significantly smaller than that of the ID samples,
% the maximum \emph{inlier} class-probability $\PTr$ scores OOD samples significantly higher than ID samples.
% }
% \todoakm{Keep only one example}
% \todoakm{Would this be a candidate for including on page 2, as a quick take-away summary?}


%
\subsection{Discussion and extensions}

%\todoakm{Is it clear why small density ratio implies deeming a sample as OOD? Hari: sorry, I think at some point we flipped the ratio, but didn't change the text. Changed ``small'' to ``large''. However, we are not clear here what we mean by solving OOD detection: is it minimizing the OOD detection rate in \eqref{eqn:ood-detection-rate} or minimizing the joint risk in \eqref{eqn:ood}. For the former, the optimal rejector thresholds the density ratio.}
%or more generally, based on some cost trade-off between the max inlier conditional-class probabilty and the density ratio.
%
% Figure~\ref{fig:ood_vs_abstention} illustrates a simple setting where these conditions may be at odds with each other.
% \todoakm{I wonder if this should be merged with Figure 2; and whether this can actually be discussed earlier? Right now we are not strongly connecting the discussion of the figure to Lemma 4.1.}
%%% Commenting it out for the time-being to send in a draft for pub-approve.
% Here, we have positive and negative samples drawn from a one-dimensional truncated Gaussian distribution.
% Samples near the origin will have $\Pr( y = 1 \mid x ) \sim 0.5$, and are candidates for abstention in the L2R setting.
% Samples away from the origin will have $\Pr( x ) \sim 0$, and are candidates for abstention in the OOD setting.
% \todoakm{Edit this}

{Given the common use (and success) of the MSP for OOD detection,
it is natural to ask when it \emph{does} work. 
One setting where the MSP score will match the Bayes classifier is for all samples $x$, 
(i) one of the classes has a sufficiently $\Pr^*(y \mid x)$, and 
(ii) when it is the unseen class that receives the highest conditional probability, all other classes have near-equal and small probability, i.e.: $\Pr^*(y \mid x) \approx \frac{\beta}{\alpha + \beta} \cdot \frac{1}{L-1}$.}

{One may also ask whether using the maximum \emph{logit} rather than softmax probability can prove successful in the open-set setting.
Unfortunately, as this similarly does not include information about $\mathbb{P}_{\rm out}$, it can also fail;
see Appendix~\ref{app:expts-max-logit}.} 
{For the same reason, rejectors that threshold the margin between the highest and the second-highest probabilities, instead of the maximum class probability, can also fail.
The use of other L2R methods such as~\citet{Mozannar:2020} may not be successful either, because the optimal solutions for these methods have the same form as MSP.}
% \todoakm{Talk about thresholding based on probability margin?}
% \todoakm{Other surrogates fail} 

% \todo{What is $\Pte$? Do we mean $\mathbb{P}_{\rm out}$?}



% }
% {
% \color{blue}
% TODO: Add intuition for when Chow may fail
% }

%
\if 0
{\bf \color{Maroon}Remark}. 
Observe that if $\Pr^*( y = L \mid x ) \sim 1$, then $\PTr( x ) \sim 0$.
Intuitively, this is because $\Pr^*( y = L \mid x ) \sim 1$ happens only if $\Pr^*( x \mid y = L ) \cdot \pi^*( L ) \sim \Pr^*( x )$,
which in turn means that either the other $\pi^*( y ) \sim 0$ or $\Pr^*( x \mid y ) \sim 0$.
This means that rejecting samples based on their training density could have some merit.
%
\fi
\if 0
{\bf \color{Maroon}Question}. 
Suppose we use a learning to reject loss, so that we estimate $\PTr( y \mid x )$ only when the latter has sufficiently high mass on the highest scoring label.
Does this help make the MSP classifier better aligned with the Bayes-optimal one?
\defcitealias{}{}
%
{\bf \color{Maroon}Question}. 
Intuitively, $\pi^*( L )$ should factor into any analysis.
But it appears missing in the above?
\wj{Isn't $\pi^*(L)$ included in $\mathbb{P}^*( y \neq L \mid x )$?}
\fi

==> coupled_ce.tex <==
\subsection{Coupled objective}
\label{app:coupled}
Another natural objective learns logits $\bar{f} \colon \XCal \to \Real^{L + 1}$ so as to minimise~\citep{Thulasidasan:2021}
\begin{align*}
    R_{\rm cce}( \bar{f} ) &= \pi_{\rm in} \cdot \mathbb{E}_{( x, y ) \sim \mathbb{P}_{\rm in}}\left[ \ell_{\rm ce}( y, \bar{f}( x ) ) \right] + (1 - \pi_{\rm in}) \cdot \mathbb{E}_{x \sim \mathbb{P}_{\rm out}}\left[ \ell_{\rm ce}( \perp, \bar{f}( x ) ) \right] \\
    &= \mathbb{E}_{( x, \bar{y} ) \sim \mathbb{P}_{\rm comb}}\left[ \ell_{\rm ce}( \bar{y}, \bar{f}( x ) ) \right],
\end{align*}
where $\pi_{\rm in}$ is the fraction of inliers versus outliers, and $\mathbb{P}_{\rm comb}$ is a mixture over inliers and outliers given by
\begin{alignat*}{2}
    \mathbb{P}_{\rm comb}( \bar{y} ) &= \pi_{\rm in} \cdot \mathbb{P}_{\rm in}( \bar{y} ) &&\text{ if } \bar{y} \neq \perp \\
    \mathbb{P}_{\rm comb}( \bar{y} ) &= 1- \pi_{\rm in} &&\text{ if } \bar{y} = \perp \\
    \mathbb{P}_{\rm comb}( x \mid \bar{y} ) &= \mathbb{P}_{\rm in}( x \mid \bar{y} ) &&\text{ if } \bar{y} \neq \perp \\
    \mathbb{P}_{\rm comb}( x \mid \bar{y} ) &= \mathbb{P}_{\rm out}( x ) &&\text{ if } \bar{y} = \perp.
\end{alignat*}
%\wj{$\mathbb{P}_{\rm comb}( \bar{y} ) = \pi_{\rm in} $?}
Here, we will obtain probabilities $\bar{p}^*_{\bar{y}}( x ) = \Pr_{\rm comb}( \bar{y} \mid x )$,
which simplifies to
\begin{align*}
    \Pr_{\rm comb}( \bar{y} \mid x ) &= \frac{\Pr_{\rm comb}( x \mid \bar{y} ) \cdot \Pr_{\rm comb}( \bar{y} )}{\Pr_{\rm comb}( x )} \\
    &= \begin{cases}
        \Pr_{\rm in}( \bar{y} \mid x ) \cdot \frac{\Pr_{\rm in}( x )}{\Pr_{\rm comb}( x )} \cdot {\pi_{\rm in}} &\text{ if } \bar{y} \neq \perp \\
        \frac{\Pr_{\rm out}( x )}{\Pr_{\rm comb}( x )} \cdot {(1 - \pi_{\rm in})} &\text{ if } \bar{y} = \perp.
    \end{cases}
\end{align*}
Observe that $\Pr_{\rm comb}( \perp \mid x )$ estimates a transformation of the likelihood ratio $\frac{\Pr_{\rm out}( x )}{\Pr_{\rm in}( x )}$: indeed,
$$ \frac{\Pr_{\rm out}( x )}{\Pr_{\rm comb}( x )} = \frac{\Pr_{\rm out}( x )}{\pi_{\rm in} \cdot \Pr_{\rm in}( x ) + (1 - \pi_{\rm in}) \cdot \Pr_{\rm out}( x )} = \frac{\frac{\Pr_{\rm out}( x )}{\Pr_{\rm in}( x )}}{\pi_{\rm in} + (1 - \pi_{\rm in}) \cdot \frac{\Pr_{\rm out}( x )}{\Pr_{\rm in}( x )}}. $$
It is however perhaps less desirable for the regular class-probability estimates $\Pr_{\rm comb}( y \mid x )$ to be additionally modified by $\frac{\Pr_{\rm in}( x )}{\Pr_{\rm comb}( x )}$:
for inlier samples, this means that we do not actually get estimates of $\Pr_{\rm in}( y \mid x )$, unlike the previous formulation.
For this reason, we choose the de-coupled CCE objective for our plug-in algorithm.


==> icml2023/abstract.tex <==
% Learning to reject (L2R) is a classical problem where a classifier is allowed to \emph{abstain} from predicting on ``hard'' samples. 
% Out-of-distribution (OOD) detection is another classical problem, wherein the goal is to detect ``anomalous'' samples not drawn from the training distribution.
% Learning to reject (L2R) is a classical problem where a classifier is allowed to \emph{abstain} from predicting on ``hard'' samples. 
% Out-of-distribution (OOD) detection is another classical problem, wherein the goal is to detect ``anomalous'' samples not drawn from the training distribution.
Learning to reject (L2R) and out-of-distribution (OOD) detection are two classical problems, 
each involving the detection of certain abnormal samples: 
% each with the goal of detecting certain abnormal samples:
% in L2R, the goal is to detect ``hard'' samples on which to abstain, 
% while in OOD detection, 
% the goal is to detect ``outlier'' samples not drawn from the training distribution. 
{the goal is to detect ``hard'' samples on which to abstain in L2R,
and 
``outlier'' samples not drawn from the training distribution in OOD detection.}
% from the same distribution as the training set.
% Intriguingly, while both problems share a simple baseline 
% ---
% the \emph{maximum softmax probability} (MSP) score
% ---
% there is limited understanding of precisely how these problems relate.
Intriguingly, despite being developed in parallel literatures, both problems share a simple baseline:
the \emph{maximum softmax probability} (MSP) score.
% While this points at a deep connection between these problems,
% there is limited formal understanding of .
% However,
Despite this connection,
there is limited understanding of precisely how these problems relate.
In this paper, we formally relate these problems, and show how they may be jointly solved.
% In particular,
% we show that popular L2R methods such as 
% % Chow's rule, 
% MSP,
% although widely used as baselines for OOD detection,
We first show that 
while MSP is theoretically optimal for L2R,
it can be \emph{sub-optimal} for OOD detection
% can be sub-optimal 
in some important settings. 
We then characterize    the Bayes-optimal classifier for a unified formulation that generalizes both L2R and OOD detection. 
Based on this, we design a  plug-in approach for learning to abstain on both inlier and OOD samples, while constraining the total abstention budget.
Experiments on benchmark OOD datasets demonstrate that our approach yields competitive classification and OOD detection performance 
% at different abstention rates 
compared to baselines from both literatures.

% AKM: I think this point is a bit too technical for the abstract
% These problems are similar in spirit, and share some common baselines, but fundamentally involve 
% identifying different samples: 
% the former involves finding samples with near-uniform conditional label density, while the latter involves finding samples with low marginal input density.
% %; in the latter, one typically trains weaker models to abstain on “hard” samples, but there is no accommodation for whether or not a sample is OOD.
% In this paper, we show that popular L2R methods such as Chow's rule, although widely used as baselines for OOD detection, can be sub-optimal in some important practical settings. 
% We then provide a characterization of the Bayes-optimal classifier for a unified formulation that generalizes both L2R and OOD detection. 
% Using the form of optimal classifier, we design a  plug-in approach for learning to abstain on both inlier and OOD samples, while constraining the total abstentions to be within a budget. 
% Experiments on benchmark OOD datasets demonstrate that our approach yields competitive classification and OOD detection performance at different abstention rates compared to baselines in both  literatures.


==> icml2023/background.tex <==
Given instances $\XCal$, labels $\YCal \defEq [ L ]$, and a distribution $\Pr$ over $\XCal \times \YCal$,
% \todoakm{Should we use $\Pr^*$? Hari: I tried doing this, but looks like we would then have to define Chow's rule in terms of $\Pr^*$, which may later become confusing when we talk about why Chow's rule fails in the open-set setting.}
multi-class classification concerns learning a classifier $h \colon \XCal \to \YCal$ with minimal misclassification error 
$R_{\rm err}( h ) \defEq \Pr( y \neq h( x ) )$.
% $R( h ) \defEq \Pr( y \neq h( x ) )$.
% \todoakm{Consistent notation: R in this section vs L in later sections. Hari: I think we use R to denote 0-1 errors, and L to denote surrogate objectives.}
Such a classifier is typically implemented via $h( x ) = \argmax_{y \in [L]} f_y( x )$,
where $f \colon \XCal \to \Real^L$ scores the affinity of each label to a given instance.
One typically learns $f$ from a training sample $S = \{ ( x_n, y_n ) \}_{n \in [N]}$ drawn from $\Pr$,
via minimisation of the \emph{empirical risk}
% $ \hat{R}( f ) = \frac{1}{N} \sum_{n \in [N]} \ell( y_n, f( x_n ) ) $
% $ \hat{R}( f; \ell ) = \frac{1}{N} \sum_{n \in [N]} \ell( y_n, f( x_n ) ) $
$ \hat{R}( f; \ell ) \defEq \frac{1}{N} \sum_{n \in [N]} \ell( y_n, f( x_n ) ) $
for \emph{loss} $\ell \colon [ L ] \times \Real^L \to \Real_+$.

% We now review the problems of learning to reject (L2R), and out-of-distribution (OOD) detection.

%
\subsection{Learning to reject (L2R)}

Standard classification assumes one makes a prediction on \emph{all} samples,
regardless of how confident the model is.
In the \emph{learning to reject} (\emph{L2R}) setting, one has the option of \emph{abstaining} from making a prediction (denoted by predicting $\perp$), at the expense of incurring a cost $c_0 \in [ 0, 1 ]$~\citep{Bartlett:2008}.
% In real-world deployment of machine learning classifiers,
Intuitively, one may wish to abstain on ``hard'' (e.g., ambiguously labelled) samples,
which could then be forwarded to an expert (e.g., a human labeller).

% \proposal{
Formally, one 
seeks to learn 
% $h \colon \XCal \to \YCal \cup \{ \perp \}$ to
classifier $h \colon \XCal \to \YCal$
and \emph{rejector} $r \colon \XCal \to \{ 0, 1 \}$,
where $r( x ) = 1$ denotes ``rejected'' samples where we abstain from making a prediction.
Our goal is
to
minimise the \emph{abstention-aware misclassification error}:
% \todoakm{Should we use $\bar{h}$ here and elsewhere?}
% \todoakm{Or should we have an explicit rejector for easy comparison to the OOD detector? Hari: I think a separate rejector may be better here. Later when we use an augmented classifier in the joint learning section, let's use $\bar h$}
\begin{equation}
    \label{eqn:abstention-aware-risk}
    % \resizebox{0.9\linewidth}{!}{$\displaystyle
    % R_{\rm rej}( h ) \defEq \Pr( y \neq h( x ), h( x ) \neq \perp ) + c_0 \cdot \Pr( h( x ) = \perp ).
    R_{\rm rej}( h, r ) \defEq \Pr( y \neq h( x ), r( x ) = 0 ) + c_0 \cdot \Pr( r( x ) = 1 ).
    % $}
\end{equation}
Intuitively, this is the standard misclassification error on non-rejected samples,
plus the cost $c_0$ times the fraction of rejected samples.
The \emph{Bayes-optimal} 
% classifier 
rejector
% --- i.e., the classifier which minimises this quantity --- 
minimising~\eqref{eqn:abstention-aware-risk}
follows \emph{Chow's rule}~\citep{Chow:1970,Ramaswamy:2018}:
\begin{equation}
    \label{eqn:chow}
    % \resizebox{0.9\linewidth}{!}{$\displaystyle
    % h^*( x ) = 
    % \begin{cases}
    %     \underset{y \in [L]}{\argmax} \, \Pr(y \mid x) & \text{if}~\underset{y \in [L]}{\max} \, \Pr(y \mid x) > 1 - c_0 \\
    %     \perp & \text{else}.
    % \end{cases}
    % h^*( x ) = 
    % \begin{cases}
    %     \underset{y \in [L]}{\argmax} \, \Pr(y \mid x) & \text{if}~r^*( x ) = 0 \\
    %     \perp & \text{else}.
    % \end{cases}    
    r^*( x ) = \indicator{ {\max}_{y \in [L]} \, \Pr(y \mid x) < 1 - c_0 }.
    % $}
\end{equation}
Intuitively, 
we abstain on ``hard'' samples where 
the most likely label is ambiguous,
i.e., it has low $\Pr( y \mid x )$.
% }
% the most likely label
% has insufficiently high probability under $\Pr( y \mid x )$;
% i.e., this label is ambiguous.

% Intuitively, 
% we only make the 
% standard prediction of the most likely label
% when this label has sufficiently high probability under $\Pr( y \mid x )$;
% i.e., this label is sufficiently unambiguous.
% We abstain on other samples, which may be deemed ``hard''.
% we abstain on samples which are ``hard'', 
% in the sense of the class probability distribution $\Pr( y \mid x )$ being insufficiently peaked on the most likely label;
% on other samples, we make the .

{Chow's rule~\eqref{eqn:chow} 
is not directly practical, since it requires knowledge of $\Pr( y \mid x )$.
The simplest L2R baseline is the \emph{confidence-based} method~\citep{Ni:2019}, 
which applies Chow's rule to a \emph{plug-in estimate} $\hat{\Pr}(y \mid x)$ of $\Pr(y \mid x)$:
given a scorer $f \colon \XCal \to \Real^L$ learned from a training sample, 
one computes softmax probability estimates $\hat{\Pr}(y \mid x) \propto \exp( f_y( x ) )$.
Samples with $\max_{y \in [L]} \hat{\Pr}(y \mid x) < 1 - c_0$ are then rejected.
Alternatively, one may modify the training loss $\ell$ to yield a consistent estimate of Chow's rule~\citep{Bartlett:2008,Ramaswamy:2018,Charoenphakdee:2021,Gangrade:2021},
or
learn an explicit rejection function jointly with the classifier~\citep{CorDeSMoh2016,Thulasidasan:2019,Mozannar:2020}.}
% The decoupling in the latter may be beneficial in settings where the base classifier has a weak capacity.

% \delete{Given a scorer $f \colon \XCal \to \Real^L$ learned from training sample $S$ using a suitable loss function, 
% one may approximate this rule using probability estimates $p_y( x ) \propto \exp( f_y( x ) )$ in place of the unknown $\Pr( y \mid x )$~\citep{Ni:2019}.}
% \todoakm{If we are including 2.3, then that already covers Ni et al.}
% \delete{One may alternately seek to directly learn $f \colon \XCal \to \Real^{L + 1}$, with an additional rejection score $f_\perp( x )$,
% and suitably modify the loss function to encourage this score to be high for low-confidence samples~\citep{Bartlett:2008,Cortes:2016,Thulasidasan:2019,Mozannar:2020,Charoenphakdee:2021}.
% Given such a scorer, we abstain iff $f_{\perp}( x ) > \max_{y' \in [ L ]} f_{y'}( x )$.}
% \todoakm{We could consider omitting this, and perhaps just say there are other approaches that modify the training? We don't seem to use the details later.}
% \todoakm{If we include, should we use $\bar{f}$?}


%
\subsection{Out-of-distribution (OOD) detection}

The out-of-distribution (OOD) detection problem concerns distinguishing instances from an 
``inlier'' distribution $\Pr_{\rm in}$
and 
an ``outlier'' distribution $\Pr_{\rm out}$~\citep{Hendrycks:2017}.
This is a natural auxiliary task in real-world deployment of machine learning classifiers,
owing to the possibility of such models producing high-confidence predictions even on completely arbitrary inputs~\citep{Nguyen:2015,Hendrycks:2017}, and scoring outlier samples higher than inlier samples~\citep{Nalisnick:2019}.
% Indeed, even models purporting to produce density estimates may incorrectly assign higher density to OOD compared to inlier samples~\citep{Nalisnick:2019}.

Formally, one seeks a binary OOD detector $r \colon \XCal \to \{ 0, 1 \}$ that predicts whether or not a given sample comes from $\Pr_{\rm out}$, so as to minimise the \emph{OOD detection error}
% \todoakm{Any better name?}
% \todoakm{Should we make it so that $r( x ) = 1( r( x ) \leq t )?$}
% \todoakm{Would $\alpha, \beta$ be clearer? Hari: I have replaced these costs with macros so that we can change them easily. Currently, changed them to $\alpha$ and $\beta$.}
% \todoakm{Should we make the costs sum to $1$? Hari: this would be problematic later on, when we combine this with the classification error, and further, set the costs to be Lagrange multipliers.}
\begin{equation}
    \label{eqn:ood-detection-rate}
    R_{\rm ood}( r ) \defEq \costin \cdot \Pr_{\rm in}( r( x ) = 1 ) + \costout \cdot \Pr_{\rm out}( r( x ) = 0 ),
\end{equation}
for suitable constants $\costin, \costout \in [0, 1]$.
This is a \emph{cost-sensitive} misclassification error~\citep{Elkan:2001}, where samples from the outlier (inlier) distribution are treated as positive (negative).
% \todoakm{Swapped positive and negative?}
% By allowing these costs to be \emph{distribution-dependent},
% one may capture a broad class of non-decomposable performance measures for binary classification, such as 
% false positive rate at 95\% true positive rate, a metric popular in the OOD detection literature~\cite{Hendrycks:2019}.
% the F-score~\citep{Narasimhan:2015b}.
One may learn $r$ by 
% first learning 
suitably thresholding
an \emph{OOD scorer}
% \todoakm{Now we are using $r$ for L2R and OOD. Different symbol?}
$s \colon \XCal \to \Real$, 
% and then suitably thresholding 
to give $r( x ) = \indicator{s( x ) < t}$. 
Via standard results~\citep{Scott:2013}, the Bayes-optimal detector for 
\eqref{eqn:ood-detection-rate} 
thresholds the \emph{density ratio} 
$\frac{\Pr_{\rm in}( x )}{\Pr_{\rm out}( x )}$:
% $g^*( x ) = \indicator{r^*( x ) \geq \frac{\alpha}{\beta}}$
% for \emph{density ratio} $r^*(x) = \frac{\Pr_{\rm out}( x )}{\Pr_{\rm in}( x )}$.
\begin{equation}
    \label{eqn:bayes-ood-detector}
    r^*( x ) = \indicator{\frac{\Pr_{\rm in}( x )}{\Pr_{\rm out}( x )} < \frac{\beta}{\alpha}}.
\end{equation}

% The costs $\costin$ and $\costout$ may be chosen to achieve a desired trade-off between the false positive and false negative rates. 
A popular metric for evaluating OOD detection methods is the fraction of outlier samples misclassified when 95\% of inlier samples are classified as inlier \cite{Hendrycks:2019, Bitterwolf:2022}. 
Minimizing this evaluation metric is equivalent to minimizing \eqref{eqn:ood-detection-rate} for suitable (possibly distribution-dependent) choices of $\costin$ and $\costout$.

% \todoakm{One critique may be that the OOD literature usually employs metrics like AUC or FPR95. For the latter, maybe we can mention somewhere that it is equivalent to a CS objective with distribution-dependent costs. Hari: added a para above. PTAL. I think we have interchanged the positives and negatives in this paper for OOD detection.}

% \delete{As an alternative to~\eqref{eqn:ood},
% one may also seek to minimise the \emph{pairwise disagreement} of $r$:
% \todoakm{Unless we use this, perhaps we can omit.}
% \begin{align*}
%     R_{\rm ood}( r ) &\defEq \mathbb{E}_{x \sim \Pr_{\rm in}} \mathbb{E}_{x' \sim \Pr_{\rm out}} \indicator{ r( x ) > r( x' ) }.
% \end{align*}
% This is one minus the area under the ROC curve of $r$~\citep{Agarwal:2005}, again treating samples from the outlier (inlier) distribution are treated as positive (negative).}
% \delete{The corresponding Bayes-optimal scorer is
% the density ratio
% $ r^*( x ) = \frac{\Pr_{\rm out}( x )}{\Pr_{\rm in}( x )}, $
% or any non-decreasing transformation thereof.}
% \todoakm{Do we use this anywhere?}


%
\begin{figure*}[!t]
    \centering
    
    \resizebox{0.97\linewidth}{!}{
        \subfigure[Uniform outlier distribution $\Pr_{\rm out}$.]{
            \includegraphics[scale=0.1825]{figs/ood_vs_abstention_v2.pdf}%
        }
        \qquad
        \subfigure[Open-set classification.]{
            \label{fig:chow-fail-example-open-set}
            % \includegraphics[scale=0.27]{figs/chow_failure_synthetic.pdf}
            \includegraphics[scale=0.27]{figs/chow_failure_synthetic_v2.pdf}
            \includegraphics[scale=0.27]{figs/max_inlier_prob_synthetic.pdf}
        }
    }
    
    \vspace{-5pt}
    \caption{
Example of two settings 
where the maximum softmax probability (MSP) baseline fails for OOD detection.
Setting {\bf (a)} considers
\emph{low-density OOD detection},
where
positive and negative samples drawn from a one-dimensional Gaussian distribution.
Samples \emph{away} from the origin will have $\Pr( x ) \sim 0$, 
and are thus outliers under the Bayes-optimal OOD detector.
However,
the MSP baseline will deem
samples \emph{near} the origin to be outliers,
as these have maximal 
% $\Pr( y = 1 \mid x ) \sim 0.5$.
$\max_{y} \Pr( y \mid x )$.
This illustrates the distinction between abstentions favoured by L2R 
(low label certainty)
and 
OOD detection 
(low density).
    % Samples \emph{near} the origin will have $\Pr( y = 1 \mid x ) \sim 0.5$, and are candidates for abstention in the L2R setting.
    % Samples \emph{away} from the origin will have $\Pr( x ) \sim 0$, and are candidates for abstention in the OOD setting.
Setting {\bf (b)} considers    
\emph{open-set classification}
where there are $L = 4$ total classes, with the fourth class 
(denoted by ${\color{red} \blacktriangledown}$)
assumed to comprise outliers not seen during training.
    Each class-conditional is an isotropic Gaussian (left).
    % The Bayes-optimal score for the OOD samples tends to be significantly smaller than that of the ID samples (middle).
    Note that
    the maximum \emph{inlier} class-probability $\PTr( y \mid x )$ scores OOD samples significantly \emph{higher} than ID samples (right).    
    Thus, 
    the MSP baseline,
    which
    declares samples with low $\max_{y} \PTr( y \mid x )$ as outliers,
    will perform poorly.
% Example of the distinction between abstention decisions for learning to reject, and OOD detection.
    }
    \label{fig:chow-fail-synthetic-example}
    \vspace{-5pt}
\end{figure*}



The viability of 
OOD detection is strongly determined by the nature of the training data.
There are three canonical settings considered in the literature:
(i) 
% In the most challenging setting, 
one only observes samples from $\Pr_{\rm in}$, and has no information on $\Pr_{\rm out}$;
% ~\citep{Hendrycks:2017};
% A popular relaxation of this setting involves 
(ii)
one
observes samples from $\Pr_{\rm in}$, and some \emph{training outlier} distribution $\Pr'_{\rm out}$;
% ~\citep{Hendrycks:2019,Thulasidasan:2021};
(iii)
% A third setting involves 
one observes samples from $\Pr_{\rm in}$, and an \emph{unlabeled mixture} of samples from $\Pr_{\rm in}$ and $\Pr_{\rm out}$.
% ~\citep{Bitterwolf:2022}.

{A remarkably effective baseline for OOD detection that requires only inlier samples is 
the \emph{maximum softmax probability}~\citep{Hendrycks:2017}, possibly with temperature scaling and data augmentation~\citep{Liang:2018}.
Given a scorer $f \colon \XCal \to \Real^L$ learned from inlier samples alone, 
one computes softmax probability estimates $\hat{\Pr}_{\rm in}(y \mid x) \propto \exp( f_y( x ) )$.
% to train a standard softmax-based probabilistic classifier,
% and use  as the OOD score $r$.
Samples with $\max_{y \in [L]} \hat{\Pr}_{\rm in}(y \mid x) < \frac{\beta}{\alpha}$ are then deemed to be OOD.
Recent works found that the maximum \emph{logit} (without softmax normalisation) may be preferable in some settings~\citep{vaze2021open,Hendrycks:2022}, possibly with normalisation~\citep{Wei:2022}.
These may be recovered as a limiting case of energy-based approaches~\citep{Liu:2020b}.}


==> icml2023/chow_suboptimal.tex <==
% {We now show that the L2R and OOD problems share a common baseline.
% While this points at a connection between the problems, we show that this baseline may \emph{fail} for some important special cases of OOD detection.}

{We now show that the L2R and OOD problems share a common baseline;
however, 
this baseline may \emph{fail} for some important special cases of OOD detection.}


% We now take a closer look at the L2R and OOD detection problems, by establishing that the MSP baseline may \emph{fail} for the latter in some important special cases.

%
% \subsection{The maximum softmax probability baseline}
% \subsection{Common baseline: maximum softmax probability}
\subsection{Maximum softmax probability meets Chow's rule}

% While largely studied independently, both L2R and OOD detection share a simple yet effective baseline:
% given a scorer $f \colon \XCal \to \Real^L$ learned from training sample $S$ using a suitable loss function, 
% one computes softmax probability estimates $p_y( x ) \propto \exp( f_y( x ) )$.
% Samples with small maximum probability $\max_{y \in [L]} p_y( x )$
% are then adjudged to be worthy of abstention, or likely outliers.
% This baseline is 
% known as \emph{Chow's rule}~\citep{Chow:1970} in the L2R literature,
% % \todoakm{Nit: Chow's rule refers to the population rule. This is more like plugin Chow. I think Ni et al. just calls it confidence-based rejection. Hari: Chow seems a bit more specific than confidence-based rejection. In any case, we are now mainly using MSP to refer to this baseline.}
% and 
% the \emph{maximum softmax probability} (\emph{MSP}) score~\citep{Hendrycks:2017} in the OOD detection literature.
% % This baseline identifies samples for which the maximum softmax probability falls below a threshold, and either abstains on them (in the case of L2R) or declares them as OOD.

{
For inlier and outlier distributions $\Pr_{\rm in}, \Pr_{\rm out}$,
consider the L2R problem on $\Pr_{\rm in}$ and OOD detection on $\Pr_{\rm in}, \Pr_{\rm out}$.
We begin with an intriguing observation:
while developed in parallel strands of literature,
the \emph{confidence-based L2R baseline and maximum softmax probability OOD baseline are identical}.
Indeed, both baselines involve learning probability estimates 
$\hat{\Pr}_{\rm in}(y|x)$,
% $p_y( x )$, 
% \todoakm{Should we distinct $\Pr$ vs $\Pr_{\rm in}$?}
and using the score $\max_{y \in [L]} \hat{\Pr}_{\rm in}(y|x)$ to determine whether to reject a sample, or deem it OOD.

Does this imply that one may similarly employ other L2R methods for OOD detection, and vice-versa?
Conceptually,
L2R and OOD detection appear related:
both problems
% abstains from predicting on certain samples.
seek to identify certain ``abnormal'' samples.
However, 
% the reason for abstention is subtly different,
the notion of ``abnormal'' is subtly different,
as may be seen from their Bayes-optimal solutions~\eqref{eqn:chow},~\eqref{eqn:bayes-ood-detector}:
in L2R, 
% it is for samples where 
we identify samples where
% $\Pr_{\rm in}( y \mid x )$ is insufficiently peaked,
$\max_{y \in [L]} \Pr_{\rm in}( y \mid x )$ is small,
while in OOD detection,
% In the OOD detection problem, it is for 
we identify
samples where 
$\frac{\Pr_{\rm in}( x )}{\Pr_{\rm out}( x )}$ is small.
% the density ratio 
% $\frac{\Pr_{\rm out}( x )}{\Pr_{\rm in}( x )}$ 
% is large.

The absence of any consideration of $\Pr_{\rm out}( x )$ in L2R suggests 
the two problems may not be interchangeable after all.
% What, then, explains the popularity of the MSP baseline?
However, despite sharing a common baseline, {and the two problems generally acknowledged to be related \citep{yang2021generalized}}, there is surprisingly limited understanding of how precisely they relate to (and differ from) each other.
% Revisiting the formulations in \S\ref{sec:background},
% any such relation must involve further assumptions:
% the L2R problem involves a single distribution, while the OOD detection problem involves both an inlier and outlier distribution.

We now show that in two special cases of OOD detection (which impose specific assumptions on $\Pr_{\rm out}$),
the MSP baseline can be strongly \emph{sub-optimal} for OOD detection.}

% As a first step towards better relating the two problems, we show that the MSP baseline
% can in fact be suboptimal for a special case of OOD detection, known as \emph{open-set classification}~\citep{Scheirer:2013}, wherein the OOD samples come from an unseen class.
% \todoakm{Maybe MSP will be a more intuitive choice of name, rather than Chow's rule? Hari: changed here and elsewhere in this section}


%
\subsection{MSP may fail for uniform $\Pr_{\rm out}$}

As a warm-up, we first consider
\emph{density-based OOD detection}, 
where we assume $\XCal \subset \Real^D$ and $\Pr_{\rm out}$ is uniform.
Assuming
without loss of generality
that the volume of $\mathscr{X}$ is normalised to $1$,
the density ratio $\frac{\Pr_{\rm in}( x )}{\Pr_{\rm out}( x )} = {\Pr_{\rm in}( x )}$.
Thus,
from~\eqref{eqn:bayes-ood-detector},
the Bayes-optimal
OOD detector for 
\eqref{eqn:ood-detection-rate}
is simply
% \todoakm{Consistent notation}
$$ r^*( x ) = \indicator{\Pr_{\rm in}( x ) < \frac{\beta}{\alpha}}; $$
that is, we deem \emph{low-density} samples to be OOD.
By contrast, the MSP baseline deems samples where 
$\max_{y \in [L]} \Pr_{\rm in}( y \mid x ) < t$ to be OOD;
% \todoakm{Is it confusing that we now use $\Pr_{\rm in}$ rather than $\Pr$?}
that is, we deem \emph{low label-certainty} samples to be worthy of abstention.

% {Recall that the
% Bayes-optimal OOD detector for 
% \eqref{eqn:ood-detection-rate} 
% is
% $g^*( x ) = \indicator{r^*( x ) \geq \frac{\alpha}{\beta}}$
% for {density ratio} $r^*(x) = \frac{\Pr_{\rm out}( x )}{\Pr_{\rm in}( x )}$.
% % Suppose that $\Pr_{\rm out}$ is uniform over $\mathscr{X}$, 
% % and 

% Then,
% the optimal detector is simply $g^*( x ) = \indicator{\Pr_{\rm in}( x ) \leq \frac{\beta}{\alpha}}$;
% that is, we deem \emph{low-density} samples to be OOD.
% By contrast, recall that the Bayes-optimal L2R rule rejects samples where $\max_{y \in [L]} \Pr_{\rm in}( y \mid x ) < t$;
% \todoakm{$\Pr$ vs $\Pr_{\rm in}$}
% that is, we deem \emph{high label-uncertainty} samples to be worthy of abstention.

How well do these two rules align?
Observe that their decisions are based on fundamentally different quantities:
the marginal density $\Pr_{\rm in}( x )$,
and the class-probability $\Pr_{\rm in}( y \mid x )$.
Consequently, it is not hard to see that these rules might be at odds:
for a fixed joint distribution $\Pr_{\rm in}( x, y )$,
one may independently vary $\Pr_{\rm in}( x )$ and $\Pr_{\rm in}( y \mid x )$
such that low marginal {density} corresponds to \emph{high} {label-certainty}.
% Thus, MSP may make predictions that are completely at odds with the Bayes-optimal predictor;
Figure~\ref{fig:chow-fail-example} illustrates this in a simple one-dimensional setting.

The above makes precise 
observations that are implicit in prior work (e.g.,~\citet{Liu:2020b}),
% \proposal{and serves as an instructive warm-up}:
% \proposal{but may appear unsurprising}, 
% as it imposes a highly specific structure on $\Pr_{\rm out}$. 
{but may appear to be an artifact of the highly specific structure assumed on $\Pr_{\rm out}$.}
% as it imposes a highly specific structure on $\Pr_{\rm out}$. 
% that may not arise in practice.
% \proposal{it hints at a key distinction between L2R and OOD detection.}
% \todoakm{In light of previous work, can perhaps downplay claimed novelty/significance; say this is just a warm-up}
{However, we now show that 
even in OOD detection settings that appear tailored to MSP,
the latter can fail.}
% We now show that a similar result holds in a practically relevant setting.
% \todoakm{Restate: MSP seems more intuitive here}


%
% \subsection{Bayes-optimal open-set classification}
\subsection{MSP may fail for open-set classification}
\label{sec:chow-fail-open-set}

Our second setting is 
\emph{open-set classification}~\citep{Scheirer:2013}, 
wherein the OOD samples come from an unseen class.
% In \emph{open-set classification},
For example, suppose
the inlier distribution $\Pr_{\rm in}$ has support on all but one class $\YCal' = \YCal - \{ L \}$,
and the outlier distribution $\Pr_{\rm out}$ has support on the remaining class $L$.
We wish to reject samples from the unseen class at test time.
Formally, suppose the underlying distribution over samples from both the known and unseen classes is $\mathbb{P}^*( x, y ) = \pi^*( y ) \cdot \mathbb{P}^*( x \mid y )$.
The outlier distribution is $\Pr_{\rm out}( x ) = \Pr^*(x \mid y=L)$,
while
the training distribution is
% given by
\begin{align*}
    \PTr( x \mid y ) = \mathbb{P}^{*}( x \mid y )
    \quad
    \piTr( y ) = \frac{1( y \neq L )}{1 - \pi^*( L )} \cdot \pi^*( y ). 
    % \\
    %
    % \PTr( x \mid y ) &= \mathbb{P}^{*}( x \mid y ).
    %
\end{align*}
That is, the class-conditional distribution remains unchanged, but we rescale the label frequencies to only exclude the contribution of the unseen label.

% With this, we may derive the following.
% \todoakm{If needed we could omit this, since it is perhaps not of independent interest, and is just a means to proving Lemma 3.2, 3.3.}

% %
% \begin{lemma}
% \label{lemm:open-set-distribution}
% For the open-set setting with notional distribution $\Pr^*$ over all labels,
% the training distribution has
% \begin{align*}
%         %
%         \PTr( x, y ) &= \frac{1( y \neq L ) }{1 - \pi^*( L )} \cdot \mathbb{P}^*( x, y ) \\
%         %
%         \PTr( x ) &= \frac{\mathbb{P}^*( y \neq L \mid x )}{1 - \pi^*( L )} \cdot \mathbb{P}^*( x ) \\
%         %
%         \PTr( y \mid x ) &= \frac{1( y \neq L )}{\mathbb{P}^*( y \neq L \mid x )} \cdot \mathbb{P}^*( y \mid x ).
%     \end{align*}
% \end{lemma}

{
% \color{blue}
Now suppose our goal is to minimize the OOD detection error~\eqref{eqn:ood-detection-rate} for suitable $\alpha, \beta$.
% We have the following optimal detector.
The optimal detector is as follows.

%%% Commented by Hari -- move to appendix?
% Under this setting, the following optimises the OOD detection rate~\eqref{eqn:ood-detection-rate}.
% \begin{lemma}
% \label{lemm:bayes-open-set-ood}
% Under the open-set setting, the Bayes-optimal classifier for the OOD detection error $R_{\rm ood}( r ) \defEq \costin \cdot \Pr_{\rm in}( r( x ) = 1 ) + \costout \cdot \Pr_{\rm out}( r( x ) = 0 )$  takes the form:
% $$
% r^*(x) = 1
%     \,\iff\,
% \mathbb{P}^*( y = L \mid x ) \geq t_{\rm OPT},
% $$
% where $t_{\rm OPT} \defEq \frac{ \costin }{ \costin + \costout}$.
% \end{lemma}
%%%
\begin{lemma}
\label{lemm:bayes-open-set-rewrite}
 Under the open-set setting, the Bayes-optimal classifier for the OOD detection error 
%  $R_{\rm ood}( r ) \defEq \costin \cdot \Pr_{\rm in}( r( x ) = 1 ) + \costout \cdot \Pr_{\rm out}( r( x ) = 0 )$  
\eqref{eqn:ood-detection-rate}
takes the form:
% \resizebox{.99\linewidth}{!}{
    % \begin{minipage}{\linewidth}
        \begin{align*}
            r^*(x) = 1
            &\iff
            \mathbb{P}^*( y = L \mid x ) \geq \frac{ \costin }{ \costin + \costout} %\\
            % &
            \iff \max_{y' \neq L} \PTr( y' \mid x ) \geq \frac{\alpha + \beta}{\beta} \cdot \max_{y' \neq L} \mathbb{P}^*( y' \mid x).
        \end{align*}
%     \end{minipage}
% }
% This can be equivalently written as:
% The Bayes-optimal classifier for the open-set setting  in Lemma \ref{lemm:bayes-open-set-ood} can be equivalently written as:
% \todoakm{Perhaps we should write $t_{\rm opt}$, or just explicitly write it in terms of $\costin, \costout$. Hari: explicitly wrote the costs.}
% $$ \max_{y' \neq L} \PTr( y' \mid x ) \geq \frac{\max_{y' \neq L} \mathbb{P}^*( y' \mid x)}{1 - t}. $$
% $$ \max_{y' \neq L} \PTr( y' \mid x ) \geq \frac{\alpha + \beta}{\beta} \cdot \max_{y' \neq L} \mathbb{P}^*( y' \mid x). $$
\end{lemma}
}

%%% Commented by Hari -- move to appendix?
% The above simply formalises a intuitive strategy: 
% samples where the true class-probability $\Pr^*( y \mid x )$ places high confidence on the unseen label $L$ are likely to be OOD.
%%%


% \subsection{When does Chow's rule fail?}

Equipped with the Bayes-optimal classifier for the open-set setting,
let us
now consider the MSP baseline,
which deems a sample to be OOD iff $\max_{y' \neq L} \PTr( y' \mid x ) < t_{\rm MSP}$ for some $t_{\rm MSP} \in [ 0, 1 ]$.
% How well does this align with the Bayes-optimal classifier for the open-set setting (Lemma~\ref{lemm:bayes-open-set-ood}), which 
% deems a sample as OOD iff $\mathbb{P}^*( y = L \mid x ) \geq t$?
Importantly, here we consider the class-probability under the \emph{inlier} distribution $\PTr$.
% since by assumption we only have access to samples from this distribution.

%%% Commented by Hari
% How well does the MSP baseline align with the optimal rule from Lemma~\ref{lemm:bayes-open-set-rewrite}?
% Surprisingly, 
% \todoakm{Is it still surprising, given we already show this for the uniform case?}
% we show that %Chow's rule 
% MSP can make predictions that disagree with the optimal rule.
% \todoakm{Is this really opposite in a formal sense?}
%%% 

%%% Commented by Hari
% \begin{lemma}
% \label{lemm:bayes-open-set-rewrite}
% The Bayes-optimal classifier for the open-set setting  in Lemma \ref{lemm:bayes-open-set-ood} can be equivalently written as:
% % \todoakm{Perhaps we should write $t_{\rm opt}$, or just explicitly write it in terms of $\costin, \costout$. Hari: explicitly wrote the costs.}
% % $$ \max_{y' \neq L} \PTr( y' \mid x ) \geq \frac{\max_{y' \neq L} \mathbb{P}^*( y' \mid x)}{1 - t}. $$
% $$ \max_{y' \neq L} \PTr( y' \mid x ) \geq \frac{\alpha + \beta}{\beta} \cdot \max_{y' \neq L} \mathbb{P}^*( y' \mid x). $$
% \end{lemma}
%%%

% {\hari{Should we delete the equation below? It looks like just the original form of Chow's rule above is clear enough to point out the difference with the Bayes-optimal classifier}
% \color{red}
% To better understand this, observe that Chow's rule equally rejects iff:
% \begin{align*}
%     % \mathbb{P}_{\rm ood}( x ) &= \mathbb{P}^*( y = L \mid x ) \\
%     % \max_{y \neq L} \PTr( y \mid x ) < t &\iff \max_{y \neq L} \mathbb{P}^*( y \mid x ) < t \cdot ( 1 - \mathbb{P}^*( y = L \mid x ) ) \\
%     % &\iff \max_{y \neq L} \mathbb{P}^*( y \mid x ) < t - t \cdot \mathbb{P}^*( y = L \mid x ) \\
%     % &\iff t \cdot \mathbb{P}^*( y = L \mid x ) < t -\max_{y \neq L} \mathbb{P}^*( y \mid x ) \\
%     % &\iff 
%     \mathbb{P}^*( y = L \mid x ) < 1 - \frac{1}{t} \cdot \max_{y \neq L} \mathbb{P}^*( y \mid x ).
% \end{align*}
% }

%That is, we reject when the probability of the unseen class is
% That is, we reject when the maximum probability is
% \emph{lower} than some threshold.

On close inspection at both the classifiers, one can see that MSP can 
make predictions that 
starkly disagree with the optimal rule. More specifically, 
Lemma~\ref{lemm:bayes-open-set-rewrite} shows that the optimal decision is to reject when the maximum softmax probability (with respect to $\PTr$) is \emph{higher} than some (sample-dependent) threshold.
This is however the precise \emph{opposite} of the MSP baseline, which rejects when the maximum probability is
\emph{lower} than some threshold.
% \begin{align*}
% \max_{y' \neq L} \PTr( y' \mid x ) < t_{\rm MSP}.
% \end{align*}

What is the reason for this stark discrepancy?
% \todoakm{Maybe some of this can be pushed to Discussion}
Intuitively, the issue is that we would like to threshold the maximum of $\Pr^*( y \mid x )$, \emph{not} $\PTr( y \mid x )$;
however, these two distributions may not align,
as the latter includes a normalisation term that causes unexpected behaviour when we threshold.
% \todoakm{Change the markers}
We illustrate this with a concrete example (see also Figure~\ref{fig:chow-fail-example-open-set}). %

%
\textbf{Example (failure of MSP baseline)}.
Consider a setting where the class probabilities $\Pr^*( y' \mid x )$ are equal for all the known classes $y' \ne L$.
% Due to the normalization term, the inlier class probabilities then evaluates to become 
This implies that
$\PTr( y' \mid x ) = \frac{1}{L-1}, \forall y' \ne L$.
The Bayes-optimal classifier rejects a sample when 
% $\Pr^*( L \mid x ) > t_{\rm OPT}$.
$\Pr^*( L \mid x ) > \frac{\alpha}{\alpha + \beta}$.
% \todoakm{Since we reference the Bayes classifier here, I brought back the lemma we moved to the appendix, and merged it with Lem 3.1.}
On the other hand,
MSP rejects a sample 
iff the threshold 
$t_{\rm MSP} < \frac{1}{L-1}$.
% $t < \frac{1}{L-1}$.
Notice that rejection decision is \emph{independent} of the unknown class density $\Pr^*( L \mid x )$, 
and therefore will not agree with the Bayes-optimal classifier in general.
% Figure \ref{fig:chow-fail-example} illustrates this with examples of two open-set settings, where the inlier class probabilities are identical, but the unknown class probability varies across samples.

The following lemma formalizes the above observation.
% \todoakm{If needed maybe we can omit this; the point is clear enough at this stage I think. Hari: the only reason why a formal statement will be helpful is because we have two different thresholds, and we wish to say no matter what threshold we choose for MSP, one can always construct a distribution where it is at odds with the Bayes classifier.}
%
%
% {
% %\color{blue}
% The following lemma formalizes the above observation to show the existence of distributions where Chow's rule disagrees with the Bayes classifier.
\begin{lemma}
Suppose the MSP baseline is implemented as  $\max_{y \neq L} \PTr( y \mid x ) < t_{\rm MSP}$ for $t_{\rm MSP} \in (0, 1)$. 
Then for any choice of $t_{\rm MSP}$, there exists an underlying conditional-class distribution $\Pr^*(y \mid x)$ for which the Bayes-optimal classifier 
$\mathbb{P}^*( y = L \mid x ) \geq t$ disagrees with MSP $\forall t \in (0, 1)$.
\label{lem:chow-fail}
\end{lemma}

% \todoakm{Add an intuitive example where Chow's rule fails. Hari: added Fig \ref{fig:chow-fail-example}.}

% \todoakm{Add results on a synthetic problem where Chow's rule fails? Hari: good idea, will get to this soon after wrapping up current set of experiments}

% \todoakm{Given this is a common baseline that seems to work reasonably, can we identify settings where Chow's rule would work as expected? Hari: one setting where Chow will match the Bayes classifier is for all samples $x$, (i) one of the classes has a sufficiently $\Pr^*(y|x)$, and (ii) when it is the unseen class that receives the highest conditional probability, all other classes have near-equal and small probability, i.e.: $\Pr^*(y|x) \approx \frac{\beta}{\alpha + \beta} \cdot \frac{1}{L-1}$}

% %
% {
% \textbf{Example (illustration of failure of MSP baseline)}.
% Figure~\ref{fig:chow-fail-synthetic-example} presents a simple two-dimensional synthetic example where the maximum softmax probability fails.
% Here, while the Bayes-optimal score for the OOD samples tends to be significantly smaller than that of the ID samples,
% the maximum \emph{inlier} class-probability $\PTr$ scores OOD samples significantly higher than ID samples.
% }
% \todoakm{Keep only one example}
% \todoakm{Would this be a candidate for including on page 2, as a quick take-away summary?}


%
\subsection{Discussion and extensions}

%\todoakm{Is it clear why small density ratio implies deeming a sample as OOD? Hari: sorry, I think at some point we flipped the ratio, but didn't change the text. Changed ``small'' to ``large''. However, we are not clear here what we mean by solving OOD detection: is it minimizing the OOD detection rate in \eqref{eqn:ood-detection-rate} or minimizing the joint risk in \eqref{eqn:ood}. For the former, the optimal rejector thresholds the density ratio.}
%or more generally, based on some cost trade-off between the max inlier conditional-class probabilty and the density ratio.
%
% Figure~\ref{fig:ood_vs_abstention} illustrates a simple setting where these conditions may be at odds with each other.
% \todoakm{I wonder if this should be merged with Figure 2; and whether this can actually be discussed earlier? Right now we are not strongly connecting the discussion of the figure to Lemma 4.1.}
%%% Commenting it out for the time-being to send in a draft for pub-approve.
% Here, we have positive and negative samples drawn from a one-dimensional truncated Gaussian distribution.
% Samples near the origin will have $\Pr( y = 1 \mid x ) \sim 0.5$, and are candidates for abstention in the L2R setting.
% Samples away from the origin will have $\Pr( x ) \sim 0$, and are candidates for abstention in the OOD setting.
% \todoakm{Edit this}

{Given the common use (and success) of the MSP for OOD detection,
it is natural to ask when it \emph{does} work. 
One setting where the MSP score will match the Bayes classifier is for all samples $x$, 
(i) one of the classes has a sufficiently $\Pr^*(y \mid x)$, and 
(ii) when it is the unseen class that receives the highest conditional probability, all other classes have near-equal and small probability, i.e.: $\Pr^*(y \mid x) \approx \frac{\beta}{\alpha + \beta} \cdot \frac{1}{L-1}$.}

{One may also ask whether using the maximum \emph{logit} rather than softmax probability can prove successful in the open-set setting.
Unfortunately, as this similarly does not include information about $\mathbb{P}_{\rm out}$, it can also fail;
see Appendix~\ref{app:expts-max-logit}.} 
{For the same reason, rejectors that threshold the margin between the highest and the second-highest probabilities, instead of the maximum class probability, can also fail.
The use of other L2R methods such as~\citet{Mozannar:2020} may not be successful either, because the optimal solutions for these methods have the same form as MSP.}
% \todoakm{Talk about thresholding based on probability margin?}
% \todoakm{Other surrogates fail} 

% \todo{What is $\Pte$? Do we mean $\mathbb{P}_{\rm out}$?}



% }
% {
% \color{blue}
% TODO: Add intuition for when Chow may fail
% }

%
\if 0
{\bf \color{Maroon}Remark}. 
Observe that if $\Pr^*( y = L \mid x ) \sim 1$, then $\PTr( x ) \sim 0$.
Intuitively, this is because $\Pr^*( y = L \mid x ) \sim 1$ happens only if $\Pr^*( x \mid y = L ) \cdot \pi^*( L ) \sim \Pr^*( x )$,
which in turn means that either the other $\pi^*( y ) \sim 0$ or $\Pr^*( x \mid y ) \sim 0$.
This means that rejecting samples based on their training density could have some merit.
%
\fi
\if 0
{\bf \color{Maroon}Question}. 
Suppose we use a learning to reject loss, so that we estimate $\PTr( y \mid x )$ only when the latter has sufficiently high mass on the highest scoring label.
Does this help make the MSP classifier better aligned with the Bayes-optimal one?
\defcitealias{}{}
%
{\bf \color{Maroon}Question}. 
Intuitively, $\pi^*( L )$ should factor into any analysis.
But it appears missing in the above?
\wj{Isn't $\pi^*(L)$ included in $\mathbb{P}^*( y \neq L \mid x )$?}
\fi

==> icml2023/conclusion.tex <==
We have thus provided a general framework that unifies L2R and OOD detection, and proposed a plug-in classifier for learning to jointly abstain on both inlier and OOD samples. 
While our analysis builds on the MSP baseline,
it is worth noting that there are many other 
effective OOD detection approaches;
in future work, it would be of interest to further study the viability of augmenting these approaches with a L2R capability.
For example, these
include approaches based on $k$-nearest neighbour~\citep{Sun:2022},
the likelihood ratio against a background sample~\citep{Ren:2019},
and methods that use a sample of ``outliers'' to train softmax based classifiers~\citep{Dhamija:2018,Chen:2021}.
%% Commented out and just retaining citations we haven't already mentioned before.
% In settings where one also has ``exposure'' to a sample of outliers,
% a simple strategy is to encourage the predicted probabilities on these samples to be uniform~\citep{Dhamija:2018,Hendrycks:2019}.
% One may also treat these samples as belonging to a separate ``outlier'' class, and use this to train a standard softmax based classifier~\citep{Thulasidasan:2021,Chen:2021}.
% A recent strategy of~\citet{Bitterwolf:2022} proposed to instead learn an explicit binary discriminator to distinguish inlier and outlier samples.
%
% It would also be of interest to \emph{improve} the OOD generalization of the learned classifier,
% and study if this may additionally help in identifying samples worthy of rejection.

% One application of proposed approach is in
% %One application of the L2R paradigm is in 
% \emph{adaptive inference}, where inference cost scales with the inherent ``difficulty'' of a sample~\citep{Bolukbasi:2017}.
% This may be achieved via early-exit models, wherein at pre-specified intermediate computation points (e.g., intermediate layers), one decides whether or not to make a prediction, or defer to the next computation point~\citep{Scardapane:2020}.
% An interesting area for exploration is equipping early-exit models with the ability to perform OOD detection, so that one may ``give up'' early on samples that are OOD, rather than redundantly forward them to the final exit.


==> icml2023/coupled_ce.tex <==
\subsection{Coupled objective}
\label{app:coupled}
Another natural objective learns logits $\bar{f} \colon \XCal \to \Real^{L + 1}$ so as to minimise~\citep{Thulasidasan:2021}
\begin{align*}
    R_{\rm cce}( \bar{f} ) &= \pi_{\rm in} \cdot \mathbb{E}_{( x, y ) \sim \mathbb{P}_{\rm in}}\left[ \ell_{\rm ce}( y, \bar{f}( x ) ) \right] + (1 - \pi_{\rm in}) \cdot \mathbb{E}_{x \sim \mathbb{P}_{\rm out}}\left[ \ell_{\rm ce}( \perp, \bar{f}( x ) ) \right] \\
    &= \mathbb{E}_{( x, \bar{y} ) \sim \mathbb{P}_{\rm comb}}\left[ \ell_{\rm ce}( \bar{y}, \bar{f}( x ) ) \right],
\end{align*}
where $\pi_{\rm in}$ is the fraction of inliers versus outliers, and $\mathbb{P}_{\rm comb}$ is a mixture over inliers and outliers given by
\begin{alignat*}{2}
    \mathbb{P}_{\rm comb}( \bar{y} ) &= \pi_{\rm in} \cdot \mathbb{P}_{\rm in}( \bar{y} ) &&\text{ if } \bar{y} \neq \perp \\
    \mathbb{P}_{\rm comb}( \bar{y} ) &= 1- \pi_{\rm in} &&\text{ if } \bar{y} = \perp \\
    \mathbb{P}_{\rm comb}( x \mid \bar{y} ) &= \mathbb{P}_{\rm in}( x \mid \bar{y} ) &&\text{ if } \bar{y} \neq \perp \\
    \mathbb{P}_{\rm comb}( x \mid \bar{y} ) &= \mathbb{P}_{\rm out}( x ) &&\text{ if } \bar{y} = \perp.
\end{alignat*}
%\wj{$\mathbb{P}_{\rm comb}( \bar{y} ) = \pi_{\rm in} $?}
Here, we will obtain probabilities $\bar{p}^*_{\bar{y}}( x ) = \Pr_{\rm comb}( \bar{y} \mid x )$,
which simplifies to
\begin{align*}
    \Pr_{\rm comb}( \bar{y} \mid x ) &= \frac{\Pr_{\rm comb}( x \mid \bar{y} ) \cdot \Pr_{\rm comb}( \bar{y} )}{\Pr_{\rm comb}( x )} \\
    &= \begin{cases}
        \Pr_{\rm in}( \bar{y} \mid x ) \cdot \frac{\Pr_{\rm in}( x )}{\Pr_{\rm comb}( x )} \cdot {\pi_{\rm in}} &\text{ if } \bar{y} \neq \perp \\
        \frac{\Pr_{\rm out}( x )}{\Pr_{\rm comb}( x )} \cdot {(1 - \pi_{\rm in})} &\text{ if } \bar{y} = \perp.
    \end{cases}
\end{align*}
Observe that $\Pr_{\rm comb}( \perp \mid x )$ estimates a transformation of the likelihood ratio $\frac{\Pr_{\rm out}( x )}{\Pr_{\rm in}( x )}$: indeed,
$$ \frac{\Pr_{\rm out}( x )}{\Pr_{\rm comb}( x )} = \frac{\Pr_{\rm out}( x )}{\pi_{\rm in} \cdot \Pr_{\rm in}( x ) + (1 - \pi_{\rm in}) \cdot \Pr_{\rm out}( x )} = \frac{\frac{\Pr_{\rm out}( x )}{\Pr_{\rm in}( x )}}{\pi_{\rm in} + (1 - \pi_{\rm in}) \cdot \frac{\Pr_{\rm out}( x )}{\Pr_{\rm in}( x )}}. $$
It is however perhaps less desirable for the regular class-probability estimates $\Pr_{\rm comb}( y \mid x )$ to be additionally modified by $\frac{\Pr_{\rm in}( x )}{\Pr_{\rm comb}( x )}$:
for inlier samples, this means that we do not actually get estimates of $\Pr_{\rm in}( y \mid x )$, unlike the previous formulation.
For this reason, we choose the de-coupled CCE objective for our plug-in algorithm.

==> icml2023/expts-plots.tex <==
\begin{figure*}[!ht]
    \centering
    
    % \resizebox{\linewidth}{!}{
        \subfigure[$\Pr_{\rm in}$: CIFAR100;~~~ $\Pr_{\rm out}$: SVHN ~~~~($\pi_{\rm mix} = 0.1$, ~~$\pi^{\rm eval}_{\rm out} = 0.25$)]{
        \includegraphics[scale=0.33]{figs/plots/icml_cf100_svhn_pi_train_0.9_pi_test_0.75.pdf}
        }
        \\[-2pt]
        \subfigure[$\Pr_{\rm in}$: CIFAR100;~~~ $\Pr_{\rm out}$: OpenImages~~~~ ($\pi_{\rm mix} = 0.5$, ~$\pi^{\rm eval}_{\rm out} = 0.5$)]{
        \includegraphics[scale=0.33]{figs/plots/icml_cf100_openimgs_pi_train_0.5_pi_test_0.5.pdf}
        }
        \\[-2pt]
        \subfigure[$\Pr_{\rm in}$: CIFAR100;~~~ $\Pr_{\rm out}$: Places365 ~~~~($\pi_{\rm mix} = 0.9$, ~$\pi^{\rm eval}_{\rm out} = 0.5$)]{
        \includegraphics[scale=0.33]{figs/plots/icml_cf100_places_pi_train_0.1_pi_test_0.5.pdf}
        } 
        \\[-2pt]
        \subfigure[$\Pr_{\rm in}$: CIFAR10;~~~ $\Pr_{\rm out}$: OpenImages; ~~~$\Pr^{\rm eval}_{\rm out}$: Places365~~~~ ($\pi_{\rm mix} = 0.1$, ~~$\pi^{\rm eval}_{\rm out} = 0.25$)]{
        \includegraphics[scale=0.33]{figs/plots/icml_cf10_opimg_eval_places_pi_train_0.9_pi_test_0.75.pdf}
        }
        \\[-5pt]
        % \includegraphics[scale=0.3]{figs/plots/cifar100_id_places_ood_pi_0.95.pdf}\\
        % \includegraphics[scale=0.3]{figs/plots/cifar100_id_places_ood_pi_0.5.pdf}\\
        % \includegraphics[scale=0.3]{figs/plots/cifar100_id_places_ood_pi_0.1.pdf}
    % }

    \caption{Plots of classification and OOD detection metrics as a function of the fraction of abstained samples (averaged over 5 trials). These include both stationary settings (a--c) with $\Pr^{\rm eval}_{\rm out} = \Pr_{\rm out}$, and a non-stationary setting with $\Pr^{\rm eval}_{\rm out} \ne \Pr_{\rm out}$, for different proportions of inlier samples $\pi_{\rm mix}$ in the unlabeled set, and different proportions of OOD samples $\pi^{\rm eval}_{\rm out}$ in the test set. 
    For the conditional risk, \emph{lower values are better}. For all other metrics, \textit{higher values are better}. 
    A `*' against a method indicates it trains on both inlier  and unlabeled samples. Higher value of $\pi_{\rm mix}$ make the unlabeled sample less reliable. 
    We set $c_{\rm ood} = 5$. In Appendix \ref{app:ranking-metrics}, we report AUC and FPR95. }
    \label{fig:expt-results}
    \vspace{-7pt}
\end{figure*}


==> icml2023/expts.tex <==
We evaluate the efficacy of the plug-in approach in solving the constrained classification task in \eqref{eqn:budget-constrainted-ood} on benchmark image classification datasets \citep{Hendrycks:2017, Bitterwolf:2022}. 
The majority of our evaluations will be on the setting described in Section \ref{sec:formulation}, where during training, we receive an unlabeled sample from $\Pr_{\rm mix} = \pi_{\rm mix} \cdot \Pr_{\rm in} + (1-\pi_{\rm mix}) \cdot \Pr_{\rm out}$, and during test time, we evaluate the classifier on a sample drawn from $\Pr^{\rm eval}_{\rm out} = \Pr_{\rm out}$. Following \citet{Katz:2022}, we also consider a variant of this setting, where the test OOD distribution is different from the one available during training, i.e., $\Pr^{\rm eval}_{\rm out} \ne \Pr_{\rm out}$. 
\input{expts-plots}

\textbf{Datasets.} We use CIFAR-10, CIFAR-100 \citep{Krizhevsky:2009} and ImageNet \citep{Deng:2009} as the inlier datasets, and SVHN \citep{netzer2011reading}, Places365 \citep{zhou2017places}, CelebA \citep{liu2015faceattributes} and OpenImages \citep{krasin2017openimages} as the OOD datasets. %We construct the training set to contain sample 50\% labeled  inlier samples and 50\% unlabeled samples. %, which could contain a mix of both inlier and OOD examples.
We train ResNet-56 on CIFAR and EfficientNet-B0 on ImageNet. See Appendix \ref{app:expts} for details about the hyper-parameter choices.

\textbf{Mixing proportions.} 
The training set we use contains 50\% labeled samples and 50\% unlabeled samples, of which $\pi_{\rm in}$ fraction of examples are inlier. We hold out 5\% of the original inlier test set and use it as the ``strictly inlier'' sample needed to estimate the proportion $\pi_{\rm mix}$ of inlier samples in the unlabeled set. 
We repeat the experiments for datasets generated with different values of $\pi_{\rm mix}$. In addition to this, we also vary the proportion $\pi^{\rm eval}_{\rm out}$ of OOD samples in the test set, a quantity we assume is known to the trainer. %: $ \frac{|S^{\rm eval}_{\rm out}|}{|S^{\rm eval}_{\rm in}| + |S^{\rm eval}_{\rm out}|}$. %We assume that $\gamma^{\rm eval}_{\rm in}$ is known \emph{apriori} during training; in practice, this may be specified by a domain expert. 

% \todo{Specify model architecture for each dataset}

\textbf{Evaluation metrics.}
Our classifiers are trained to satisfy a budget constraint on the fraction of abstentions. For a fixed proportion of abstentions, we measure both the classification and OOD detection performance using the following metrics:
\begin{align*}
    \text{inlier-acc}(\bar{h}) &= \frac{
        \sum_{(x,y) \in S_{\rm in}}\indicator{ \bar{h}(x) \ne \abstain, y = \bar{h}(x)}
        }
        {
        \sum_{x \in S_{\rm all}}\indicator{ \bar{h}(x) \ne \abstain }
        }\\
    \text{ood-precision}(\bar{h}) &= \frac{
        \sum_{(x,y) \in S_{\rm out}}\indicator{ \bar{h}(x) = \abstain}
        }
        {
        \sum_{x \in S_{\rm all}}\indicator{ \bar{h}(x) = \abstain}
        }\\
    \text{ood-recall}(\bar{h}) &= \frac{
        \sum_{x \in S_{\rm out}}\indicator{ \bar{h}(x) = \abstain}
        }
        {
        |S_{\rm out}|
        },
\end{align*}
where $S_{\rm all} = \{x: (x, y) \in S_{\rm in}\} \cup S_{\rm out}$ is the combined set of inlier and OOD instances. 
The \emph{conditional inlier accuracy} is the fraction of non-abstained samples on which the prediction was correct. The \emph{OOD precision} is the fraction of abstained samples which were OOD. The \emph{OOD recall} is the fraction of OOD samples on which the model abstained.

To measure the combined performance on the classification and OOD detection tasks, we 
additionally evaluate the \emph{OOD-weighted combined error} in \eqref{eqn:ood}. Below is a version of the metric conditioned on the non-abstained samples, and normalized to not exceed 1:
% \resizebox{0.9\linewidth}{!}{
\begin{align*}
  \lefteqn{
  \textstyle
%   \hspace{-5pt}
  \text{comb-error}(\bar{h}) =
  \frac{1}{Z}\cdot
  \Big(\sum_{(x, y) \in S_{\rm in}}\indicator{ \bar{h}(x) \ne \abstain , y = \bar{h}(x) }
  }\\
  &  
  \textstyle
  \hspace{3.5cm}
  {+~ c_{\rm ood} \cdot
        \sum_{x \in S_{\rm out}}\indicator{ \bar{h}(x) \ne \abstain }
    \Big)},
\end{align*}
% }
where
$Z = (1 + c_{\rm ood}) \cdot\sum_{x \in S_{\rm all}}\indicator{ \bar{h}(x) \ne \abstain }$. 
In all our experiments, we set $c_{\rm ood} = 5$. 
We also report ranking metrics such as AUC for the learned OOD detection scorers.

%, i.e., denoting that the cost of failing to abstain on OOD samples is five times that of making a mistake on an inlier sample.
% In each case, we evaluate the OOD-weighted risk 
% in \eqref{eqn:ood-weighted}, conditioned on the non-abstained samples:
% $\hat{\Ex}\left[\ell(y, h(x)) \,|\, h(x) \ne \perp \right]$
% from \eqref{eqn:cond-ood} 
% \begin{align*}
% \hat{\Ex}\big[
% \1(y \ne h(x)) + c_{\rm ood} \cdot \1(y = \abstain)
% \,\big|\, h(x) \ne \perp\big],
% \end{align*}

% \begin{align*}
% \frac{
% \sum_{n}\1( h(x_n) \ne \perp ) \cdot \left( \1(y_n \ne h(x_n)) + c_{\rm ood} \cdot \1(y_n = \abstain) \right)
% }
% {
% \sum_{n}\1( h(x_n) \ne \perp )
% },
% \end{align*}
% where the sample $S = \{(x_n, y_n)\}_{n \in [N]}$ comprises of both inlier and OOD examples, with label $y_n$ set to $\abstain$ for the OOD examples. We also evaluate the OOD detection rate:
% \[
% \frac{
% \sum_{n}\1( y_n = \abstain) 
% }
% {
% \sum_{n}\1( h(x_n) \ne \perp )
% }.
% \]
% \todo{Explain why the conditional doesn't effect the form of the plug-in classifier}



\textbf{Baselines.} We include  Chow's rule (or MSP) and the cost-sensitive softmax (CSS) loss of \citep{Mozannar:2020} as representative baselines from the L2R literature. Both these methods use only the inlier samples for training. 
From the OOD literature, we include both methods which train only on the inlier samples, namely,  MaxLogit \citep{Hendrickx:2021}, energy-based scorer \citep{Hendrickx:2021}, ODIN  \citep{Hendrickx:2021}, and SIRC \citep{Xia:2022}, and methods which additionally use unlabeled samples, such as the coupled CE loss (CCE) of \citet{Thulasidasan:2021}, the de-coupled CE loss (DCE) of \citet{Bitterwolf:2022}, and the outlier exposure (OE) loss of \citet{Hendrycks:2019}. The closest among these to our approach is SIRC, which also seeks to treat inlier abstentions differently from OOD abstentions, but uses a heuristic post-hoc rule.


% The following methods use only the inlier dataset:
% \begin{itemize}[itemsep=0pt,topsep=0pt,leftmargin=16pt]
%     \item \textit{MSP or Chow's rule}: Train a scorer $f: \cX \rightarrow \R^L$ using CE loss, and threshold the MSP %$\max_{y \in [L]} p_y(x)$
%     to decide to abstain \citep{Chow:1970, Hendrycks:2017}. 
%     \item \textit{MaxLogit}: Same as above, but instead threshold the maximum logit $\max_{y \in [L]} f_y(x)$  \citep{Hendrickx:2021}.
%     \item \textit{Energy score}: Same as above, but threshold the energy function $-\log\sum_y \exp(f_y(x))$
%     \citep{Liu:2020}.
%     % \item \textit{Mahalanobis score}:
% \end{itemize}
% The following  use both the inlier and unlabeled samples:
% \begin{itemize}[itemsep=0pt,topsep=0pt,leftmargin=16pt]
%     \item \textit{Coupled CE (CCE)}: Train a scorer $f \colon \XCal \to \Real^{L + 1}$, augmented with a rejection score $f_\perp( x )$ by optimizing the CCE loss of \citet{Thulasidasan:2021}, and abstain iff $f_{\perp}( x ) > \max_{y' \in [ L ]} f_{y'}( x ) + t$, for threshold $t$.
%     \item \textit{De-coupled CE (DCE)}: Same as above but uses the DCE loss of \citet{Bitterwolf:2022} for training.
%     \item \textit{Outlier Exposure (OE):} Train a scorer using the OE loss of \citet{Hendrycks:2019} and threshold the MSP.
%     % \item \textit{Cost-sensitive CE:}
% \end{itemize}
With each baseline, we tune the relevant threshold or cost parameter to achieve the desire rate of abstention on a held-out validation set (more details in Appendix \ref{app:expts}). For the plug-in method, as noted in Section \ref{sec:budget-constraint}, we vary the parameter $\lambda$ to control the amount of abstentions.
%, and plot the corresponding conditional risk and OOD detection rate metrics.

% \subsection{Stationary setting: train on $\Pr_{\mix}$ and test on $\Pr_{out}$}

\textbf{Results.}\ We present representative results in Figure \ref{fig:expt-results} for both the stationary setting, where $\Pr^{\rm eval}_{\rm out} = \Pr_{\rm out}$ ((a)--(c)), and the non-stationary setting, where $\Pr^{\rm eval}_{\rm out} \ne \Pr_{\rm out}$ (d), and include additional results in Appendix \ref{app:expts}. In each case, we plot the classification and OOD  metrics as a function of the percentage of abstained samples. 

One can see a few general trends.
The combined error decreases with more abstentions; the inlier accuracy increases with abstentions.  The OOD precision is the highest initially when the abstentions are on the OOD samples, but decreases when the OOD samples are exhausted, and the abstentions are on the inlier samples; the opposite is true for OOD recall.

%and starts to decrease when the number of abstentions exceeds the number of OOD samples in the test set (i.e., when the fraction of abstentions exceeds $\gamma^{\rm eval}_{\rm in}$). A similar trend is seen with 
%  the OOD recall, except that it is lowest initially, and increases with increasing abstentions. 

The main takeaway from these results is that, the proposed plug-in method is  competitive for most operating points.
% 
% \textbf{Stationary setting: $\Pr^{\rm eval}_{\rm out} = \Pr_{\rm out}$.} %
It yields \emph{lower or similar values in combined weighted error} compared to the baselines, while \emph{matching the best performing OOD detectors} on precision and recall. In contrast, the baselines either perform well on classification accuracy, or on the OOD metrics, but usually not on both. Perhaps unsurprisingly, the methods that only use the inlier sample for training (e.g., MSP or ODIN) fare well on the inlier accuracy, but under-perform on the OOD metrics. The methods which use the unlabeled samples for training (CCE, DCE, OE) fare well on the OOD metrics, but suffer on the inlier accuracy in the higher abstention regime. %Our  approach is seen to do well on both sets of metrics. %, as evident from its performance on the combined weighted risk.
%by it yielding comparable or lower values on the joint weighted risk compared to all other methods.

%This observation is aligned with our theoretical results in Section \ref{sec:chow-sub-optimal} showing the sub-optimality of MSP for OOD detection.

Finally, in keeping with our sub-optimality results, 
%in Section \ref{sec:chow-sub-optimal}, 
MSP is seen to under-perform on the OOD metrics. However, it is among the best performing methods on inlier accuracy in settings where $\pi_{\rm mix}$ is high (i.e., where the unlabeled training set contains a higher fraction of inlier samples). While in these high-noise settings, the plug-in approach sometimes yields a lower inlier accuracy than methods trained only on the inlier samples, it is still very competitive on the combined (weighted) error metric, indicating that it is able to do a better job of optimizing the desired trade-off between classification and OOD detection performance compared to the baselines. 
%, and  generally fares  better than other methods that use both the inlier and unlabeled data for training (indicated by a `*').

%The competitiveness of the plug-in method in the non-stationary setting, $\Pr^{\rm eval}_{\rm out} \ne \Pr_{\rm out}$ shows the robustness of the approach to changes in the OOD distribution.

% \textbf{Non-stationary setting: $\Pr^{\rm eval}_{\rm out} \ne \Pr_{\rm out}$.} Despite the evaluation OOD set being different from the one used for training, the proposed plug-in method is often competitive on both the conditional risk and the inlier accuracy, while yielding similar precision and recall. This shows robustness of 
% \begin{figure*}
% \centering
% \includegraphics[scale=0.3]{figs/plots/cifar100_id_svhn_ood_pi_0.95.pdf}\\
% \includegraphics[scale=0.3]{figs/plots/cifar100_id_svhn_ood_pi_0.5.pdf}\\
% \includegraphics[scale=0.3]{figs/plots/cifar100_id_svhn_ood_pi_0.1.pdf}
% \caption{Results on on CIFAR100 (inlier) + SVHN (OOD): Plots of conditional risk and OOD detection rates as a function of the fraction of abstained samples for varying values of inlier mixing proportion $\pi_{\rm in}$ in the training sample, and OOD penalty $c_{\rm ood}$.}
% \label{fig:cifar100-svhn}
% \end{figure*}




% \begin{figure*}
% \centering
% \includegraphics[scale=0.3]{figs/plots/cifar100_id_openimages_ood_pi_0.95.pdf}\\
% \includegraphics[scale=0.3]{figs/plots/cifar100_id_openimages_ood_pi_0.5.pdf}\\
% \includegraphics[scale=0.3]{figs/plots/cifar100_id_openimages_ood_pi_0.1.pdf}
% \caption{Results on on CIFAR100 (inlier) + OpenImages (OOD): Plots of conditional risk and OOD detection rates as a function of the fraction of abstained samples for varying values of inlier mixing proportion $\pi_{\rm in}$ in the training sample, and OOD penalty $c_{\rm ood}$.}
% \label{fig:cifar100-openimgs}
% \end{figure*}


==> icml2023/formulation.tex <==
% {
% \color{blue}
% TODO: Add motivating use-case.}
We now turn our attention to learning a classifier that minimizes the joint risk in \eqref{eqn:ood} for  user-specified costs $\costin$ and $\costout$. We adopt the setting of \citet{Katz:2022}, and assume access to a labeled inlier sample $S_{\rm in}$ % = \{(x_n, y_n)\}_{n \in [N]}$ 
drawn i.i.d.\ from $\Pr_{\rm in}$ and an unlabeled sample, $S_{\rm mix}$ %= \{x^u_n\}_{n^u \in [N^u]}$, 
consisting of a mixture of inlier and outlier samples drawn i.i.d.\ from $\Pr_{\rm mix} = \pi_{\rm mix} \cdot \Pr_{\rm in} + (1-\pi_{\rm mix}) \cdot \Pr_{\rm out}$. 
We will also assume access to a handful of examples $S^*_{\rm in}$ % = \{(x^i_n, y^i_n)\}_{n^i \in [N^i]}$ 
certified to be strictly inlier, i.e., with $\Pr_{\rm out}(x) = 0, \forall x \in S^*_{\rm in}$.

%For convenience, we assume that the test sample has equal proportions of inlier and OOD samples.
% Our goal would be to then learn a classifier an augmented classifier $h \colon \XCal \to \YCal \cup \{ \abstain \}$
% We will find it useful to define the conditional probability functions $\eta_{\rm out}(x) = \frac{ \Pr_{\rm out}(x) }{ \Pr_{\rm in}(x) +  \Pr_{\rm out}(x) }$ and $\eta_{\rm mix}(x) = \frac{ \Pr_{\rm mix}(x) }{ \Pr_{\rm in}(x) +  \Pr_{\rm mix}(x) }$.


\subsection{A plug-in classification approach}
\label{sec:plug-in}
The form of the Bayes-optimal classifier from the previous section suggests a simple two-step procedure to learning a joint classifier: (i) construct estimators for the inlier class probabilities $\Pr_{\rm in}( y \mid x )$ and the inverse density ratio $\frac{ \Pr_{\rm out}(x) }{ \Pr_{\rm in}(x) }$  using the training sample; (ii) plug estimates of these quantities into \eqref{eqn:joint-ood-bayes} to approximate the Bayes classifier.

\textbf{Surrogate minimization.} For the first step, we adopt a surrogate loss from \citet{Bitterwolf:2022}, 
to jointly estimate $\Pr_{\rm in}( y \mid x )$, and the unlabeled-to-inlier density ratio $\frac{ \Pr_{\rm mix}(x) }{ \Pr_{\rm in}(x) }$. Specifically, 
for classification logits $f \colon \XCal \to \Real^L$ and an OOD scorer $s \colon \XCal \to \Real$, we minimize:
% \todoakm{Consistency of notation $L$ vs $R$}
% \todoakm{TODO: fix everywhere, e.g., Alg 1}
\begin{align}
%  \lefteqn{L( f, r ) ~= 
\lefteqn{R_{\rm dce}( f, s ) ~= 
 \mathbb{E}_{( x, y ) \sim \mathbb{P}_{\rm in}}\left[ \ell_{\rm ce}( y, {f}( x ) ) \right]}
 \label{eqn:decoupled-surrogate}
 \\
 & + \mathbb{E}_{x \sim \mathbb{P}_{\rm in}}\left[ \ell_{\rm log}( -1, s( x ) ) \right] + \mathbb{E}_{x \sim \mathbb{P}_{\rm mix}}\left[ \ell_{\rm log}( +1, s( x ) ) \right],
 \nonumber
 \end{align}
where $\ell_{\rm ce} \colon [ L ] \times \Real^L \to \Real_+$ is the softmax cross-entropy loss and $\ell_{\rm log} \colon \{ \pm 1 \} \times \Real \to \Real_+$ is the logistic loss. In words, this the usual softmax cross-entropy loss on the inlier samples with a loss that discriminates between the inlier and the unlabeled samples.
%Such an objective was considered in~\citet{Bitterwolf:2022}.
It is easy to see that the optimal logits ${f}^*_y( x ) \propto \log(\Pr_{\rm in}( y \mid x ))$ and
$s^*( x ) = \log\left( \frac{ \Pr_{\rm mix}(x) }{ \Pr_{\rm in}(x) } \right)$. In this step, we do not impose separate costs for the OOD detection errors, as the goal is to estimate a density ratio;  see Appendix \ref{app:coupled} for a discussion on alternate surrogate losses.
% \footnote{One may similarly employ the coupled CE loss of \citet{Thulasidasan:2021} for this joint estimation step; we explain in Appendix \ref{app:coupled} why the objective we choose is better suited for our purpose.}
%Further, for strictly proper composite $\ell_{\rm bin}$, the optimal $r^*( x ) = \psi\left( \eta_{\rm mix}(x) \right)$, where $\psi: [0, 1] \rightarrow \R$ is the associated link function. 
% \todoakm{Should we comment up-front why the costs are not featuring in the objective? Added a note at the end -- was not entirely sure how to begin with this.}

Let $\hat{f}$ and $\hat{s}$ denote the logits and OOD scorer obtained by minimizing the objective in \eqref{eqn:decoupled-surrogate} with samples $S_{\rm in}$ and $S_{\rm mix}$; we then have estimates
 $\hat{\Pr}_{\rm in}(y|x) \propto \exp( \hat{f}_y(x))$ for the inlier class probabilities, and estimate $\exp(\hat{s}(x))$ for  $\frac{ \Pr_{\rm mix}(x) }{ \Pr_{\rm in}(x) }$.

\textbf{Density ratio transformation.} %The learned OOD scorer only gives us an estimator for  $\frac{ \Pr_{\rm mix}(x) }{ \Pr_{\rm in}(x) }$. 
To translate our estimate for $\frac{ \Pr_{\rm mix}(x) }{ \Pr_{\rm in}(x) }$ to that for $\frac{ \Pr_{\rm out}(x) }{ \Pr_{\rm in}(x) }$, we apply a simple transformation:
% Given estimates for $\eta_{\rm mix}(x)$, we can estimate $\eta_{\rm out}(x)$ by leveraging the following result.
\begin{lemma} For any $\pi_{\rm mix} < 1,$
$$
    \frac{ \Pr_{\rm out}(x) }{ \Pr_{\rm in}(x) } =  \frac{1}{1-\pi_{\rm mix}} \cdot \left( \frac{ \Pr_{\rm mix}(x) }{ \Pr_{\rm in}(x) } - \pi_{\rm mix} \right).
$$
\label{lem:wild-noise-correction}
\vspace{-0.5cm}
\end{lemma}
The above transformation requires knowing the mixing proportion $\pi_{\rm mix}$ of inlier samples in the unlabeled dataset. To estimate $\pi_{\rm mix}$, we observe that for a example $x$ that is deemed to be strictly inlier, i.e., for which $\Pr_{\rm out}(x) = 0$, we have  $\frac{ \Pr_{\rm mix}(x) }{ \Pr_{\rm in}(x)} = \pi_{\rm mix}$. Therefore, using the small sample $S^*_{\rm in}$ of strictly inlier examples, we can  estimate $\hat{\pi}_{\rm mix} = \frac{1}{|S^*_{\rm in}|}\sum_{x \in S^*_{\rm in}} \exp(\hat{s}(x))$. The inverse density ratio can then be estimated as  $\hat{\gamma}_{\rm ood}(x) = \frac{1}{1-\hat{\pi}_{\rm mix}} \cdot \left( \exp( \hat{s}(x) ) - \hat{\pi}_{\rm mix} \right).$
%n practice, one may resort to standard techniques in the positive-unlabeled (PU) learning literature to estimate this quantity (e.g., \citet{garg2021mixture}). 
% \todo{Replace this with details of the exact procedure, which should be straight-forward}

\textbf{Plug-in classifier.} 
% Having obtained the inlier class probability estimates
%  $\hat{\Pr}_{\rm in}(y|x) \propto \exp( \hat{f}_y(x))$, % \frac{\exp( \hat{f}_y(x)) }{ \sum_{y' \in [L]} \exp( \hat{f}_{y'}(x)) }$
% and  density ratio estimates $\hat{\gamma}(x) = \frac{1}{1-\hat{\pi}_{\rm in}} \cdot \left( \exp( \hat{s}(x) ) - \hat{\pi}_{\rm in} \right)$, what 
Plugging the above estimates into \eqref{eqn:joint-ood-bayes} then gives us an approximation to the Bayes classifier:
% \todoakm{Confirm: $>$ or $<$?}
% \todoakm{Notation: use $\hat{\Pr}$ when describing Chow too?}
 \begin{align}
    \label{eqn:plugin}
    % \resizebox{0.9\linewidth}{!}{
    \displaystyle
    % \lefteqn{\hat{h}( x ) =}\\
    % &
    % \hspace{-5pt}
    % \begin{cases}
    %     \abstain & \text{if}~\underset{y \in [L]}{\max} \, \hat{\Pr}_{\rm in}(y \mid x) > 1 - \costin + \costout \cdot \hat{\gamma}_{\rm ood}(x) \\
    %     \underset{y \in [L]}{\argmax} \, \hat{f}_y(x) & \text{else}.
    % \end{cases}
    % \nonumber
    \hat{h}( x ) &=
    \begin{cases}
        \abstain & \text{if}~\underset{y \in [L]}{\max} \, \hat{\Pr}_{\rm in}(y \mid x) < \hat{t}( x ) \\
        \underset{y \in [L]}{\argmax} \, \hat{f}_y(x) & \text{else}
    \end{cases} \\
    \hat{t}( x ) &\defEq 1 - \costin + \costout \cdot \hat{\gamma}_{\rm ood}(x).
    \nonumber    
    % }
\end{align}
%  abstain when
%  \[
% \max_{y \in [L]}\hat{\Pr}_{\rm in}(y|x) < 1 - \costin + \costout \cdot \hat{\gamma}(x),
%  \]
%  and predict $\argmax_{y \in [L]}\,\hat{f}_y(x)$ otherwise.
% \todoakm{An algorithm box might be useful to summarize. Hari: done}
 We summarize the details of this procedure in
 Algorithm \ref{algo:plugin}.
 
 
 
\begin{figure}[t]
\vspace{-6pt}
\begin{algorithm}[H]
\caption{Plug-in classification algorithm}
\label{algo:plugin}
\begin{algorithmic}[1]
\STATE \textbf{Input:} Labeled set $S_{\rm in} \sim \Pr_{\rm in}$, Unlabeled set $S_{\rm mix} \sim \Pr_{\rm mix}$, Strictly inlier set $S^*_{\rm in}$ with $\Pr_{\rm out}(x) = 0, \forall x\in S^*_{\rm in}$
\\[-10pt]
\STATE \textbf{Parameters:} Costs $\costin, \costout$
\STATE \textbf{Surrogate opt:} Solve $\hat{f}, \hat{s} \in \underset{f, r}{\argmin}\, \hat{R}_{\rm dce}(f, s),$
\vspace{-10pt}
\begin{align*}
\lefteqn{
\textstyle
\text{where}~
\hat{R}_{\rm dce}(f, r) \defEq \frac{1}{|S_{\rm in}|}\sum_{(x, y) \in S_{\rm in}} \ell_{\rm ce}(y, f(x))}\\
&
\textstyle
\hspace{3cm} +  \frac{1}{|S_{\rm in}|}\sum_{(x, y) \in S_{\rm in}} \ell_{\rm log}(-1, s(x))\\
& 
\textstyle 
\hspace{3cm} + \frac{1}{|S_{\rm mix}|}\sum_{x \in S_{\rm mix}} \ell_{\rm log}(-1, s(x))
\end{align*}
\vspace{-10pt}
\STATE \textbf{Inlier class probabilities:} $\hat{\Pr}_{\rm in}(y|x) \defEq \frac{ \exp( \hat{f}_y(x)) }{ \sum_{y'} \exp( \hat{f}_{y'}(x)) }$
\STATE \textbf{Mixture proportion:} $\hat{\pi}_{\rm mix} \defEq \frac{1}{|S^*_{\rm in}|}\sum_{x \in S^{*}_{\rm in}} \exp(\hat{s}(x))$
\STATE \textbf{Density ratio:}  $\hat{\gamma}_{\rm ood}(x) \defEq \frac{1}{1-\hat{\pi}_{\rm mix}} \cdot \left( \exp( \hat{s}(x) ) - \hat{\pi}_{\rm mix} \right)$
\STATE \textbf{Plug-in classifier:} Plug estimates $\hat{\Pr}_{\rm in}(y|x)$, $\hat{\gamma}_{\rm ood}(x)$, and costs $\costin, \costout$ into \eqref{eqn:plugin}, and construct classifier $\hat{h}$
\STATE \textbf{Output:} $\hat{h}$
\end{algorithmic}
\end{algorithm}
\vspace{-16pt}
\end{figure} 
  
 
%  $\hat{\eta}_{\rm mix}(x) = \psi^{-1}( \hat{r}(x) )$
% A natural question that comes up from the previous discussion  is whether there is benefit to solving the  L2R and OOD detection problems in a joint manner. More specifically, we ask how one may learn a  classifier that can abstain on both  low-confidence inlier samples and OOD samples, while minimizing the joint risk in \eqref{eqn:ood}. 
% given user-specified costs for different types of abstentions


% Turning to the
%  Bayes-optimal classifier  for the joint objective, we notice that there are two key statistics that need to estimated: the inlier class probabilities and the inlier-OOD density ratio. Fortunately, recent surrogate losses allow us to jointly train classification and OOD logits to estimate both these  quantities \citep{Thulasidasan:2021, Bitterwolf:2022}. One can then readily plug in these estimates into the form of the Bayes-optimal classifier to construct an approximation to it.


% Our observations from the previous sections suggest that
% when training an OOD-aware classifier, it is important that we specify explicit penalties for both abstentions on both inlier samples and OOD samples. In some applications, we may want the classifier to abstain on only the OOD samples, while in others, we may additionally allow for abstentions on  some low-confidence inlier samples.

% A convenient way to have a practitioner provide these different requirements could be through specification of a budget on the total proportions of abstentions, and additionally a cost for failing to abstain on OOD samples. This way the classifier is encouraged to abstain on OOD samples, and can use the the remaining budget to also abstain on ``hard'' inlier samples. We now use the form of the Bayes-optimal classifier from the previous section to construct a plug-in classifier for this joint constrained learning problem.

% To showcase the utility of this plug-in based approach, we consider a practical application where one specifies a budget on the total proportions of abstentions, and additionally, the cost for failing to abstain on OOD samples. The abstention budget may be based on the monetary expenditure involved in forwarding the abstained samples to an expert, and the OOD cost may be indicative of the extent to which making a prediction on an OOD sample is worse than a mistake on an inlier sample. Both these specifications are intuitive for  a practitioner to provide, and have the effect of encouraging a  classifier to abstain first on OOD samples, and then use the remaining budget  to abstain on ``hard'' inlier samples. 
% \todo{Argue why this formulation is natural}

\subsection{Incorporating budget constraints}
\label{sec:budget-constraint}
 In practice, it may be more natural for a user to specify a  budget on the total amount of abstentions, rather than a cost $\costin$ on the inlier abstention rate. Our formulation easily accommodates this change. More formally, suppose we want to learn a classifier $\bar{h}: \XCal \rightarrow [L] \cup \{\abstain\}$ to solve:
 \begin{align}
%   \lefteqn{
%   \hspace{-2cm}
   \min_{\bar{h}}\,   \Pr_{\rm in}( y \neq \bar{h}( x ), \bar{h}( x ) \neq \abstain )  + c_{\rm ood} \cdot \Pr_{\rm out}( \bar{h}( x ) \neq \abstain ) \quad
%   } 
%   \nonumber\\
    % \alpha_{\rm in} \cdot \Pr_{\rm in}( h( x ) = \abstain ) + (1 - \alpha_{\rm in}) \cdot \Pr_{\rm out}( h( x ) = \abstain )  \leq B_{\rm abs},
    % & 
    \text{s.t.}~~\Pr^*( \bar{h}( x ) = \abstain )  \leq B_{\rm abs},
    \label{eqn:budget-constrainted-ood}
\end{align}
where $\Pr^*(x) = (1 - \pi_{\rm out})\cdot \Pr_{\rm in}(x) + \pi_{\rm out}\cdot\Pr_{\rm out}(x)$ denotes the target distribution with known proportions of inlier and OOD samples, $B_{\rm abs} \in [0, 1]$ is the abstention budget, and $c_{\rm ood} \in \Real_+$ is the cost for failing to abstain on OOD samples. 
For a large cost $c_{\rm ood}$, this constrained problem encourages a  classifier {to abstain first on OOD samples, and then use the remaining budget  to abstain on ``hard'' inlier samples}. 

Appealing to Lagrangian theory, we can show that the above problem is equivalent to minimizing the  joint error in \eqref{eqn:ood} for a particular choice of the cost parameters. 
%One can then readily apply the approach in the previous section to learn a plug-in classifier for the problem. The specifics of the Lagrangian formulation is provided in Appendix \ref{app:lagrangian}.
\begin{align*}
    % \Pr_{\rm in}( y \neq h( x ) ) \,+\, \\
    % \lefteqn{
    % \hspace{-0.3cm}
    \Pr_{\rm in}( y \neq \bar{h}( x ), \bar{h}( x ) \neq \abstain ) + \lambda \cdot (1 - \pi_{\rm out}) \cdot \Pr_{\rm in}( \bar{h}( x ) = \abstain ) 
    % } 
    % \\
    % \nonumber
    % &\hspace{2.2cm}
    + (c_{\rm ood} - \lambda \cdot \pi_{\rm out}) \cdot \Pr_{\rm out}( \bar{h}( x ) \neq \abstain ),
\end{align*}
for Lagrange multiplier $\lambda \in \Real_+$.
%(details in Appendix \ref{app:constrained-to-costs}).
% \begin{lemma}
% Suppose the density ratio  $\frac{ \Pr_{\rm out}(x) }{ \Pr_{\rm in}(x) }$ is absolutely continuous w.r.t.\ $x$. Then there exists a value of $\lambda \in \Real_+$ for which minimizing the following joint risk yields the  Bayes-optimal classifier for \eqref{eqn:budget-constrainted-ood}:
% \begin{align*}
%     % \Pr_{\rm in}( y \neq h( x ) ) \,+\, \\
%     \lefteqn{
%     \hspace{-0.5cm}
%     \Pr_{\rm in}( y \neq h( x ), h( x ) \neq \abstain ) + \lambda \cdot \Pr_{\rm in}( h( x ) = \abstain ) } \\
%     \nonumber
%     &\hspace{2.2cm}
%     + (c_{\rm ood} - \lambda) \cdot \Pr_{\rm out}( h( x ) \neq \abstain ).
% \end{align*}
% \end{lemma}
%
%

Note that for any fixed $\lambda$, we can use the procedure in the Section \ref{sec:plug-in} to construct a plug-in classifier that minimizes the above joint risk. Finding the optimal $\lambda$ then reduces to an inexpensive threshold search. %, as we show in detail in Appendix \ref{app:constrained-to-costs}. 
% To see this, note that 
% the Bayes-optimal classifier (from Lemma \ref{lem:ood-bayes}) for the above joint risk uses the following abstention rule: abstain on $x$ when
% \[
% \frac{1}{1 +\frac{ \Pr_{\rm out}(x) }{ \Pr_{\rm in}(x) }} \cdot \left(1 - \max_{y \in [L]}\Pr_{\rm in}(y|x) \right)
%  + \frac{ \frac{ \Pr_{\rm out}(x) }{ \Pr_{\rm in}(x) } }{1 +\frac{ \Pr_{\rm out}(x) }{ \Pr_{\rm in}(x) }} \cdot c_{\rm ood} \geq \lambda,
% \]
% where the multiplier $\lambda$ serves as a simple threshold. 
%
In fact, we only need to  implement the surrogate minimization step of the plug-in procedure once to estimate the relevant probabilities; we can then construct multiple plug-in classifiers for different values of $\lambda$, and choose among those satisfying the budget constraint,  the one that minimizes the objective in \eqref{eqn:budget-constrainted-ood}.



% One can then carry out a sweep over $\lambda$,  constructing a plug-in classifier for each value, and choosing among the learnt classifiers that satisfy the budget constraint in \eqref{eqn:budget-constrainted-ood},  the one that minimizes the cost-weighted objective. Note that this one-dimensional parameter sweep can be implemented efficiently by running the first step of the plug-in procedure (surrogate minimization) only once, and repeating plug-in step  alone for different values of $\lambda$. The latter is inexpensive to implement as it involves simply re-calculating the equation for the Bayes classifier.

% Before closing, we point out that 
\textbf{Remark.} The previous work of \citet{Katz:2022} also seeks to solve an optimization problem with explicit constraints on abstention rates. However, there are some subtle, but important, technical differences between their formulation and ours, which we explain in Appendix \ref{app:katz-samuels}.

% For convenience, we assume that the underlying population %$\Pr^*$  contains equal proportions of inlier and OOD samples.
% , with the inlier examples labeled with the ground truth label $y \in [L]$ and the OOD examples labeled with $\abstain$. 
% % We would then like to evaluate the classifier $h$ against the following combine distribution:
% % \begin{align*}
% %     \Pcomb(x) &= \frac{\Pr_{\rm in}( x ) +  \Pr_{\rm out}( x )}{ 2 }.
% % \end{align*}
% We would like to learn a classifier $h: \XCal \rightarrow [L] \cup \{\perp\}$, augmented with an abstain option $\perp$.  Given a cost $c_{\rm ood}$ for making a valid prediction on an OOD sample, we measure the performance of the classifier through its \emph{conditional cost-sensitive} risk on the non-abstained samples:
% % \begin{align}
% %     \lefteqn{R_{\rm cond}(h) = } \nonumber\\
% %     &~
% %     \frac{
% %         \Pr_{\rm in}( y \neq h( x ),\, h( x ) \neq \perp )  + c_{\rm ood} \cdot \Pr_{\rm out}( h( x ) \neq \perp )
% %     }{
% %         2. \left(\Pr_{\rm in}( h( x ) \ne \perp ) + \Pr_{\rm out}( h( x ) \ne \perp )\right)
% %     }.
% %     \label{eqn:cond-ood}
% % \end{align}
% \begin{align}
%     {R_{\rm cond}(h) = } 
%     &~
%     \Ex_{(x,y) \sim \Pr^*}\left[\ell_{\rm ood}(y, h(x)) \,|\, h(x) \ne \perp \right],
%     \label{eqn:cond-ood}
% \end{align}
% where
% \begin{align*}
% \lefteqn{\ell_{\rm ood}(y, h(x)) = 
% \1(y \ne h(x), h(x) \ne \perp)}\\ 
% & \hspace{3cm} + c_{\rm ood} \cdot \1(y = \abstain, h(x) \ne \perp).
% \end{align*}
%
\if 0
We would like to learn a classifier $h: \XCal \rightarrow [L] \cup \{\perp\}$, augmented with an abstain option $\perp$.  Given a cost $c_{\rm ood}$ for failing to abstain on a OOD sample, we measure the classifier's OOD-weighted risk on the non-abstained samples:
\begin{align}
    \lefteqn{ R_{\rm ood}(h) = \Pr_{\rm in}( y \neq h( x ), h( x ) \neq \perp ) }
    \nonumber
    \\
    & \hspace{3.5cm} + c_{\rm ood} \cdot \Pr_{\rm out}( h( x ) \neq \perp ).
    \label{eqn:ood-weighted}
\end{align}
In words, on the samples that the classifier makes a valid prediction, we assign a penalty of 1 for mistakes on inlier examples and a penalty of $c_{\rm ood}$ if the example happens to be OOD. %Note that the cost $c_{\rm ood}$ is indicative of the extent to which failure to abstain on an OOD sample is worse than a mistake on an inlier sample.

Our goal is to then minimize $R_{\rm ood}$
 subject to a budget constraint on total proportion of abstentions:
\begin{align}
    \lefteqn{\min_{h: \XCal \rightarrow [L] \cup \{\perp\}} R_{\rm ood}(h)} \nonumber\\
    \text{s.t.}~~ &
    \frac{1}{2} \cdot \left( \Pr_{\rm in}( h( x ) = \perp ) + \Pr_{\rm out}( h( x ) = \perp ) \right) \leq B_{\rm abs},
    \label{eqn:budget-constrainted-ood}
\end{align}
% \begin{align}
%     \min_{h: \XCal \rightarrow [L] \cup \{\perp\}} R_{\rm ood}(h)
%     ~~\text{s.t.}~~ 
%     \Pr^*( h( x ) = \perp )  \leq B_{\rm abs},
%     \label{eqn:budget-constrainted-ood}
% \end{align}
for a budget $B_{\rm abs} \in [0, 1]$.
\fi
% Our goal is to then minimize $R_{\rm cond}$
%  subject to a budget constraint on total proportion of abstentions:
% % \begin{align}
% %     \lefteqn{\min_{h: \XCal \rightarrow [L] \cup \{\perp\}} R_{\rm cond}(h)} \nonumber\\
% %     \text{s.t.}~~ &
% %     \Pr_{\rm in}( h( x ) = \perp ) + \Pr_{\rm out}( h( x ) = \perp ) \leq 2 \cdot B_{\rm abs},
% %     \label{eqn:budget-constrainted-ood}
% % \end{align}
% \begin{align}
%     \min_{h: \XCal \rightarrow [L] \cup \{\perp\}} R_{\rm cond}(h)
%     ~~\text{s.t.}~~ 
%     \Pr^*( h( x ) = \perp )  \leq B_{\rm abs},
%     \label{eqn:budget-constrainted-ood}
% \end{align}
% for a budget $B_{\rm abs} \in [0, 1]$.

% {
% \color{blue}
% TODO: Add connection to \citet{Katz:2022}.
% }
\if 0
Under mild distributional assumptions, the above constrained optimization problem can be equivalently framed as a minimizing the joint classification risk in \eqref{eqn:ood} (via the Lagrangian for the problem), for some choice of costs $\costin$ and $\costout$. The optimal classifier for the resulting cost-weighted objective admits a closed-form solution similar to Lemma \ref{lem:ood-bayes}.
\begin{lemma}[Bayes-optimal classifier for budget-constrained OOD-aware classification]
\label{lem:ood-constrained-bayes}
Let $\eta_{\rm out}( x ) = \frac{ 1}{ 1 + \frac{ \Pr_{\rm in}(x) }{ \Pr_{\rm out}(x) }}$. Suppose the conditional distributions $\Pr_{\rm in}(y|x)$ and $\eta_{\rm out}( x )$ are absolutely continuous in $x$. 
The optimal solution to \eqref{eqn:budget-constrainted-ood} then takes the form:
\begin{align*}
    h^*(x) &= 
            \begin{cases}
                \perp & \text{if}~
                    z( x ) > t_{\rm abs}
                    \\
                \argmax_{y \in [L]}\Pr_{\rm in}(y|x) &
                \text{else}
            \end{cases}, \\
    \text{where}&~z( x ) ~\defEq
    (1 - \eta_{\rm out}(x)) \cdot \left(1 - \max_{y \in [L]}\Pr_{\rm in}(y|x) \right)\\
    &
    \hspace{4.5cm} + \eta_{\rm out}(x) \cdot c_{\rm ood},
\end{align*}
for some threshold $t_{\rm abs} \in \R_+$.
\end{lemma}

\subsection{Plug-in based solution}
We are now ready to provide a plug-in based solution to the constrained learning problem in \eqref{eqn:budget-constrainted-ood}. We adopt the same setup as \citet{Katz:2022}, and assume access to a labeled inlier sample $S = \{(x_n, y_n)\}_{n \in [N]}$ drawn i.i.d.\ from $\Pr_{\rm in}$ and an unlabeled sample $S^u = \{x^u_n\}_{n \in [N]}$, consisting of a mixture of inlier and outlier samples drawn i.i.d.\ from $\Pr_{\rm mix} = \pi_{\rm in} \cdot \Pr_{\rm in} + (1-\pi_{\rm in}) \cdot \Pr_{\rm out}$.
% We will overload notations and use $\Pin$ to denote both the joint distribution over the inlier instances and labels, and the marginal distribution over the inlier instances. 
% We consider the problem of learning a classifier $h: \XCal \rightarrow [L] \cup \{\perp\}$, that either predicts one of $L$ labels or the abstain option $\perp$. We may abstain on either the outlier examples or on examples on which $\Pr_{\rm in}(y | x)$ is not sufficiently peaked. 
%

\subsection{Formulation of \citet{Katz:2022}}
A related formulation is that of \citet{Katz:2022} which seeks to minimize the fraction of abstained examples on the OOD distribution subject to constraints on the fraction of abstained inlier examples and the error rate on the inlier examples. While they consider separate models for the base classifier and the rejector, we re-write their formulation below, with a single joint classifier $h: \XCal \rightarrow [L] \cup \{\perp\}$:
\begin{align}
   \lefteqn{
   \min_{h}~
   \Ex_{x \sim \Pout}\left[ \1\left( h(x) \ne \perp \right) \right] }
   \label{eq:ks-original}
   \\
    \text{s.t.}\hspace{10pt}
    & \Ex_{x \sim \Pin}\left[ \1\left( h(x) = \perp \right) \right] = \alpha
    \nonumber
    \\
    & \Ex_{(x, y) \sim \Pin}\left[ \1\left( h(x) \ne y,\, h(x) \ne \perp \right) \right]  = \beta,
    \nonumber
\end{align}
for some $\alpha, \beta \in (0,1)$. Here, for simplicity, we enforce an \emph{equality} in all the constraints. 

{\bf \color{Maroon}Remark}.  We calculate the inlier error rate only on examples on which the classifier predicts a base class. In the original paper, because the authors use seperate models for the base classifier and OOD detector, the inlier error rate is evaluated independent of the OOD detection decisions.

Because we may not have direct access to samples from $\Pout$, the authors suggest the following alternate formulation that instead minimizes the fraction of abstained examples on the wild distribution subject to the same constraints:
\begin{align}
   \lefteqn{\min_{h}~\Ex_{x \sim \Pwld}\left[ \1\left( h(x) \ne \perp \right) \right] }
   \label{eq:ks-reformulation}
   \\
    \text{s.t.}\hspace{10pt}
    & \Ex_{x \sim \Pin}\left[ \1\left( h(x) = \perp \right) \right] = \alpha
    \nonumber
    \\
    & \Ex_{(x, y) \sim \Pin}\left[ \1\left( h(x) \ne y,\, h(x) \ne \perp \right) \right]  = \beta.
    \nonumber
\end{align}

% To see that the formulations in \eqref{eq:ks-original} and \eqref{eq:ks-reformulation} are equivalent, notice that the objective in \eqref{eq:ks-reformulation} can be expanded:
% \[
% \Ex_{x \sim \Pwld}\left[ \1\left( h(x) \ne \perp \right) \right]
% = 
% \pi_{\rm in} \cdot \Ex_{x \sim \Pin}\left[ \1\left( h(x) \ne \perp \right) \right]
% \,+\,
% (1 - \pi_{\rm in}) \cdot \Ex_{x \sim \Pout}\left[ \1\left( h(x) \ne \perp \right) \right].
% \]
% When the fraction of abstained inlier examples are constrained to be equal to $\alpha$, we have that \[
% \Ex_{x \sim \Pwld}\left[ \1\left( h(x) \ne \perp \right) \right] = 
% \pi_{\rm in} \cdot (1-\alpha)
% \,+\,
% (1 - \pi_{\rm in}) \cdot \Ex_{x \sim \Pout}\left[ \1\left( h(x) \ne \perp \right) \right],
% \]
% which is scaled-translated form of the objective in \eqref{eq:ks-original}. 
This can easily be shown to be equivalent to~\eqref{eq:ks-original}, owing to the constraint that the fraction of abstained inlier examples is exactly $\alpha$.

{\bf \color{Maroon}Remark}. In their paper, \citet{Katz:2022} consider the same formulations with inequality constraints, and show that they are equivalent under some mild assumptions.


\subsection{Proposed formulation}
In practice, it is convenient for a practioner to the provide a budget on the fraction of inlier examples we are allowed to abstain on $\Ex_{x \sim \Pin}\left[ \1\left( h(x) = \perp \right) \right]$. 
 One may also want to have a constraint on the OOD miss rate $\Ex_{x \sim \Pout}\left[ \1\left( h(x) \neq \perp \right) \right]$. However, because we do not have direct access to outlier samples, we instead enforce a constraint on a similar miss rate computed on the wild examples $\Ex_{x \sim \Pwld}\left[ \1\left( h(x) \neq \perp \right) \right]$, which together with the constraint inlier abstention rate, implicitly constraints the OOD miss rate.
 
We  seek to solve the following constrained optimization problem:
\begin{align}
%   \lefteqn{
   &\min_{h}~\Ex_{(x, y) \sim \Pin}\left[ \1\left( h(x) \ne y,\, h(x) \ne \perp \right) \right]
%   }
   \label{eq:proposed}
   \\
    \text{s.t.}\hspace{10pt}
    & \Ex_{x \sim \Pin}\left[ \1\left( h(x) = \perp \right) \right] \leq b_{\rm in}
    \nonumber
    \\
    & \Ex_{x \sim \Pwld}\left[ \1\left( h(x) \neq \perp \right) \right]  \leq b_{\rm wild},
    \nonumber
\end{align}
where $b_{\rm in}$ and $b_{\rm wild}$ are the user-specified budgets. 

{\bf \color{Maroon}Remark}. Note that when $b_{\rm in} = 0$, the above problem reduces to that of plain OOD detection as the classifier abstains on no inlier samples. When $b_{\rm wild} = 1$, the second constraint becomes ineffective, and the problem reduces to that of learning to reject (where the cost for rejection included in the form of a budget constraint).

From the Lagrangian for the above problem, we formulate an equivalent cost-sensitive optimization problem with cost parameters $c_{\rm in}$ and $c_{\rm wild}$:
\begin{align}
  &\min_{h}~\Ex_{(x, y) \sim \Pin}\left[ \1\left( h(x) \ne y,\, h(x) \ne \perp \right) \right]
  \,+\, \\
  &c_{\rm in} \cdot
  \Ex_{x \sim \Pin}\left[ \1\left( h(x) = \perp \right) \right] 
  \,+\, \\
  &c_{\rm wild} \cdot
  \Ex_{x \sim \Pwld}\left[ \1\left( h(x) \ne \perp \right) \right],
   \label{eq:cs}
\end{align}
for costs $c_{\rm in}, c_{\rm wild} \in \R_+$.

%
% \[
% \Ex_{(x, \bar{y}) \sim \Pcomb}\left[ \1\left( \bar{y} \ne \perp,\,  h(x) \ne \bar{y},\, h(x) \ne \perp \right) 
%   \,+\,
%   c_{\rm in} \cdot
% \1\left(\bar{y} \ne \perp,\, h(x) = \perp \right) 
%   \,+\,
%   c_{\rm wild} \cdot
%   \1\left(\bar{y} = \perp,\, h(x) = \perp \right) \right]
% \]
%
To characterize the Bayes-optimal solution to the above problem, we write out the underlying combined training distribution which contains samples from $\Pr_{\rm in}$ and $\Pr_{\rm out}$ in equal proportions, and associate with each instance $x$ either a true label from $[L]$ or the outlier class, denoted by $\perp$:
\begin{align*}
    \Pcomb(x) &= \frac{\Pr_{\rm in}( x ) +  \Pr_{\rm wild}( x )}{ 2 }\\
    \eta_{\rm wild}(x) &= \frac{ \Pr_{\rm wild}(x)}{
        \Pr_{\rm in}(x) + 
        \Pr_{\rm wild}(x)}\\
    \Pcomb(\bar{y}|x) &= 
        \begin{cases}
            \eta_{\rm wild}(x) & \text{if}~\bar{y} = \perp\\
            (1 - \eta_{\rm wild}(x)) \cdot \Pr_{\rm in}( \bar{y} | x ) & \text{else}
        \end{cases}.
\end{align*}


\begin{lemma}
\label{lem:ood-wild-bayes}
The optimal solution to \eqref{eq:cs} takes the form:
\begin{align*}
    h^*(x) &= 
            \begin{cases}
                \perp & \text{if}~
                    z( x ) > 0
                    \\
                \argmax_{y \in [L]}\Pr_{\rm in}(y|x) &
                \text{else},
            \end{cases} \\
    z( x ) &\defEq (1 - \eta_{\rm wild}(x)) \cdot \left(1 - \max_{y \in [L]}\Pr_{\rm in}(y|x) - c_{\rm in }\right) \\
    & \hspace{5cm} + \eta_{\rm wild}(x) \cdot c_{\rm wild}.
\end{align*}
\end{lemma}

\subsection{Application to open-set classification}
In the special case of open-set classification described in Section \ref{sec:chow-sub-optimal}, 
we would assume access to both labeled samples drawn from the known classes (i.e., drawn from $\PTr$), and unlabeled samples from both the known and unseen classes (i.e., drawn from $\Pr^*$). More specifically, we would have:
\begin{align*}
         \Pwld(x) &= \Pr^*( x )\\
        %
        \Pcomb(x) &= \frac{\PTr( x ) +  \Pr^*( x )}{ 2 }\\
        %
        \Pcomb(\bar{y}|x) &= 
        \begin{cases}
            \frac{ \Pr^*(x)}{
                \PTr(x) + 
                \Pr^*(x)} & \text{if}~\bar{y} = \perp\\
            \frac{ \Pr_{\rm in}(x)}{
                \Pr_{\rm in}(x) + 
                \Pr^*(x)} \cdot \PTr( \bar{y} | x ) &
            \text{else}
        \end{cases}.
\end{align*}
\fi

==> icml2023/intro.tex <==
In typical classification problems, one seeks to learn a classifier that is capable of making accurate predictions on \emph{all} samples. 
However, in many real-world applications, it may be beneficial to allow the classifier to \emph{abstain} from predicting on ``hard'' (e.g., ambiguously labelled) examples. 
% at an added cost (e.g., monetary cost). 
This \emph{learning to reject} (L2R) or \emph{learning with abstention} paradigm
has been well-studied~\citep{Chow:1970, Bartlett:2008, Cortes:2016, Ramaswamy:2018, Thulasidasan:2019, Ni:2019, Charoenphakdee:2021}, 
with more recent works considering a variant where the classifier is allowed to defer to an expert~\citep{raghu2019direct, raghu2019algorithmic, Mozannar:2020,okati2021differentiable, verma2022calibrated,Narasimhan:2022}.
A distinct problem that has also received much attention is  \emph{out-of-distribution (OOD) detection}, where the goal is to detect samples that are ``outliers'',
in the sense of not being drawn from a classifier's training distribution~\citep{Hendrycks:2017, Lee:2018, Ren:2019, Bitterwolf:2022, Katz:2022}.  
A special case of this problem, referred to as \emph{open-set classification}, seeks to identify samples that belong to a class not seen during training \citep{bendale2016towards, vaze2021open}.

{While conceptually similar 
---
intuitively, it is desirable for a classifier to abstain on OOD samples
---
L2R and OOD detection have been developed in parallel literatures.}
Intriguingly, however,
% Intriguingly, while studied in parallel literatures, 
both problems share a simple yet effective baseline:
{one thresholds the maximum softmax probability from a standard classifier, with low probability samples adjudged to be abstention-worthy, or likely outliers.
This is known as 
\emph{Chow's rule}~\citep{Chow:1970} for L2R,
and
the \emph{maximum softmax probability} (\emph{MSP}) score~\citep{Hendrycks:2017} for OOD detection.}

Given this connection,
one may ask:
% This raises the natural question of 
how precisely do these problems relate, and can they be jointly solved?
{Surprisingly, 
while L2R and OOD detection are 
generally acknowledged to be related~\citep{yang2021generalized},}
these questions have 
% received limited study (see~\S\ref{sec:background}).
not received systematic study (see~\S\ref{sec:background}).
In this paper, 
% we 
% % address this issue by 
% formally study and unify 
% % the L2R and OOD detection problems,
% these problems,
% with the following contributions:
we make the following contributions towards addressing this issue:
\begin{enumerate}[label=(\roman*),itemsep=0pt,topsep=0pt]
    \item 
    We prove that the MSP baseline
    can be \emph{sub-optimal} for important special cases of OOD detection,
    such as open-set classification (\S\ref{sec:chow-sub-optimal}, Lemmas \ref{lemm:bayes-open-set-rewrite}, \ref{lem:chow-fail}).

    \item 
    We outline a formulation that unifies both the L2R and OOD detection paradigms, 
    and show that 
    the resulting Bayes-optimal classifier involves a \emph{sample-dependent threshold} on the MSP
    % the Bayes-optimal classifier for the joint learning problem intricately depends on both the inlier class probabilities and the OOD density ratio 
    (\S\ref{sec:relation}, Lemma \ref{lem:ood-bayes}). 
    
    \item  
    We propose a plug-in algorithm that seeks to approximate the Bayes classifier, and showcase its application to learning an OOD-aware classifier with a budget constraint on the total proportion of abstentions 
    (\S\ref{sec:formulation}).
    
    \item 
    Our experiments on benchmark OOD detection image datasets show that our plug-in approach yields competitive classification and OOD detection performance at any desired abstention rate, compared to both standard learning to reject and OOD detection baselines (\S\ref{sec:expts}).
\end{enumerate}

% First, we show that while Chow's rule is an optimal strategy for L2R problems,
% there exist 
% settings where it is \emph{arbitrarily sub-optimal} for OOD detection, 
% particularly in the open-set classification setting.
% % More broadly, even more recent L2R methods such the approach of \citet{Mozannar:2020} can be provably sub-optimal for OOD detection.
% % This serves as an important qualifier as to the distinction between the two problems.
% Second,
% % to more effectively solve both problems,
% we outline a formulation that unifies both the paradigms, and seeks to learn a classifier that can abstain on both low-confidence inlier samples and on OOD samples. 
% Importantly, we allow for the specification of separate cost penalties for abstaining on inlier samples (e.g., monetary cost for deferring to an expert), and for \emph{failing} to abstain on OOD samples (e.g., cost to reputation due to an embarrassingly wrong prediction). 
% % We show that the Bayes-optimal classifier for this joint learning problem depends not only on the inlier class conditionals $\Pr_{\rm in}(y|x)$, but also the density ratio $\frac{ \Pr_{\rm in}(x) }{ \Pr_{\rm out}(x) }$. 
% {As a practical application of our formulation, we show how to learn an OOD-aware classifier that satisfies a budget constraint on the total proportion of abstentions via a plug-in estimator.}


% As a practical application of our formulation, we show how to learn an OOD-aware classifier that satisfies a budget constraint on the total proportion of abstentions. Our solution is a plug-in based approach that approximates the Bayes-optimal classifier by estimating the inlier class probabilities and the density ratio. We show how these quantities can be estimated with only access to a labeled inlier dataset and an unlabeled dataset comprising of a mixture of inlier and OOD samples \citep{Katz:2022}.  


% Both the learning to reject and OOD detection settings are similar in spirit, in that one seeks to abstain on certain samples.
% At closer glance, however, 
% % they are fundamentally different in the samples they seek to identify: 
% the abstention is on fundamentally different samples:
% in the former, the goal is to abstain on samples that are  ``hard'' to classify, i.e., its conditional-class distribution is insufficiently peaked; in the latter, it is to abstain on samples from an unseen class, or more generally, from a distribution different from the training distribution.
% More formally, let $\Pr_{\rm in}(x)$ denote the marginal distribution over the ``inlier'' examples used for training, and $\Pr_{\rm in}( y \mid x )$ denote the conditional-class probability for the inlier samples. In the learning to reject setting, we abstain on sample $x$ when $\Pr_{\rm in}( y \mid x )$ is insufficiently peaked, whereas in OOD detection, we abstain on sample $x$ when $\Pr_{\rm in}(x)$ is not sufficiently large.

% Interestingly both the  literatures share some common baselines. 
% For example, in the learning to reject literature, a popular approach is Chow's rule~\citep{Chow:1970}, where one obtains  estimates $\hat{\Pr}_{\rm in}( y \mid x )$ of the inlier conditional-class probabilities, and rejects samples for which the maximum class probability $\max_{y \in [L]}\hat{\Pr}_{\rm in}( y \mid x )$ falls below a particular threshold. 
% In the OOD detection literature, the same technique, dubbed  as the max softmax probability (MSP) approach, has  been shown to be a competitive baseline for detecting OOD samples \citep{Hendrycks:2017}. 
%A variant of this approach that thresholds the maximum logit instead of the maximum softmax probability has shown to further improve detection accuracy \cite{Hendrickx:2021}.

% Our first key observation in this paper is that, while Chow's rule is an optimal strategy for abstaining on inlier samples, it can be theoretically sub-optimal when used for OOD detection, particularly in the open-set classification setting. The reason for this is that OOD detection requires identifying samples for which the density ratio $\frac{ \Pr_{\rm in}(x) }{ \Pr_{\rm out}(x) }$ is small, and  the  inlier conditional probability check that Chow's rule uses on may not always be indicative of this. For the same reason, other L2R methods such the approach of \citet{Mozannar:2020} are also sub-optimal for OOD detection.

% To better relate L2R with OOD detection, 
% we outline a formulation that unifies both the paradigms, and seeks to learn a classifier that can abstain on both low-confidence inlier samples and on OOD samples. Importantly, we allow for the specification of separate cost penalties for abstaining on inlier samples (e.g., monetary cost for deferring to an expert), and for \emph{failing} to abstain on OOD samples (e.g., cost to reputation due to an embarrassingly wrong prediction). 
% %For example, there may be a monetary cost to abstaining on an inlier sample as one might then need to defer an expert to make a prediction; similarly, predicting a class label on OOD sample may cause damages to reputation, and incur severe costs. 
% %To accommodate both these scenarios, we propose a unified formulation that assigns explicit cost penalities to both types of abstentions, and seeks to learn a classifier that optimizes for the cost trade-offs. 
% %We point out that the commonly used Chow's rule or the MSP baseline can be theoretically sub-optimal for this task. 
% We show that the Bayes-optimal classifier for this joint learning problem depends not only on the inlier class conditionals $\Pr_{\rm in}(y|x)$, but also the density ratio $\frac{ \Pr_{\rm in}(x) }{ \Pr_{\rm out}(x) }$. 

% In summary, we make the following contributions:
% \todoakm{Maybe this can replace the above para? We can include more details in each point}
% \begin{enumerate}[label=(\roman*),itemsep=0pt,topsep=0pt]
%     \item We prove that Chow's rule or the MSP baseline
%     % , which identifies samples with near-uniform class probabilities, 
%     can be sub-optimal when used for OOD detection in the open-set classification setting (\S\ref{sec:chow-sub-optimal}, Lemmas \ref{lemm:bayes-open-set-ood}--\ref{lem:chow-fail}).
%     % The same is true of other surrogate-based methods for L2R.

%     \item %Building on the work of \citet{Katz:2022}, 
%     We outline a formulation that unifies both the L2R and OOD detection paradigms, and show that the Bayes-optimal classifier for the joint learning problem intricately depends on both the inlier class probabilities and the OOD density ratio (\S\ref{sec:relation}, Lemma \ref{lem:ood-bayes}). 
    
%     \item  We propose a plug-in algorithm that seeks to approximate Bayes-optimal solution, and showcase its application to learning an OOD-aware classifier with a budget constraint on the total proportion of abstenstions % to construct a plug-in classifier from an inlier labeled sample and an unlabeled mixture of inilier and OOD samples
%     % we show how to learn a joint plug-in classifier that maximizes classification and OOD detection performance at a given abstention rate 
%     (\S\ref{sec:formulation}).
    
%     \item Our experiments on benchmark OOD detection image datasets show that our plug-in approach yields competitive classification and OOD detection performance at any desired abstention rate, compared to both standard learning to reject and OOD detection baselines (\S\ref{sec:expts}).
% \end{enumerate}

% \subsection{Related work}
% \todo{Elaborate on further related work}


==> icml2023/post_hoc.tex <==
%Building on the characterization in Lemma \ref{lem:ood-bayes}, we propose a plug-in approach to minimize the OOD-aware misclassication risk in \eqref{eqn:ood}. 
The plug-in procedure involves three steps: 
\begin{enumerate}[label=(\roman*),itemsep=0pt,topsep=0pt,leftmargin=16pt]
    \item Obtain estimates of conditional distributions $\Pr_{\rm in}(y | x)$ and $\eta_{\rm mix}(x)$ by minimizing a joint surrogate loss.
    \item Apply a correction to the estimate of $\eta_{\rm mix}(x)$ to obtain an estimate for $\eta_{\rm out}(x)$.
    \item Construct a plug-in classifier that mimics the form in Lemma \ref{lem:ood-constrained-bayes} using estimates for $\Pr_{\rm in}(y | x)$ and $\eta_{\rm out}(x)$.
\end{enumerate}

\textit{Conditional-probability estimation:} For the first step, we propose minimizing a joint classification and OOD detection objective from \citet{Bitterwolf:2022}, which for
logits $f \colon \XCal \to \Real^L$, and a scorer $r \colon \XCal \to \Real$ takes the form:
\begin{align*}
 \lefteqn{L( f, r ) ~= \mathbb{E}_{( x, y ) \sim \mathbb{P}_{\rm in}}\left[ \ell_{\rm ce}( y, {f}( x ) ) \right]}\\
 & + \mathbb{E}_{x \sim \mathbb{P}_{\rm in}}\left[ \ell_{\rm bin}( -1, r( x ) ) \right] + \mathbb{E}_{x \sim \mathbb{P}_{\rm mix}}\left[ \ell_{\rm bin}( +1, r( x ) ) \right],
 \end{align*}
where $\ell_{\rm ce} \colon [ L ] \times \Real^L \to \Real_+$ is the softmax cross-entropy and $\ell_{\rm bin} \colon \{ \pm 1 \} \times \Real \to \Real_+$ is a binary surrogate loss.
% \wj{Should the second term be $\mathbb{E}_{x \sim \mathbb{P}_{\rm in}}\left[ \ell_{\rm bin}( -1, -r( x ) ) \right]$?}
In words, we combine the usual softmax cross-entropy loss on the inlier samples with a loss that discriminates between the inlier and the unlabeled samples.
%Such an objective was considered in~\citet{Bitterwolf:2022}.
It is easy to see that the Bayes-optimal logits ${f}^*_y( x ) \propto \log(\Pr_{\rm in}( y \mid x ))$.
Further, for strictly proper composite $\ell_{\rm bin}$, the Bayes-optimal $r^*( x ) = \psi\left( \eta_{\rm mix}(x) \right)$, where $\psi: [0, 1] \rightarrow \R$ is the associated link function. One may also employ other joint objectives available in the literature, such as the coupled  cross-entropy loss of \citet{Thulasidasan:2021}.


\textit{Noise correction:} Given estimates for $\eta_{\rm mix}(x)$, we can estimate $\eta_{\rm out}(x)$ by leveraging the following result.
\begin{lemma} For any $\pi_{\rm in} < 1,$
$$
    \eta_{\rm out}(x) =  \frac{ (1 + \pi_{\rm in}) \cdot \eta_{\rm mix}(x) - \pi_{\rm in} }{2\pi_{\rm in} \cdot \eta_{\rm mix}(x) + 1 - 2\pi_{\rm in}}.
$$
\label{lem:wild-noise-correction}
\vspace{-0.5cm}
\end{lemma}
To apply the above transformation, we will need to know the mixing proportion $\pi_{\rm in}$ of inlier samples in the unlabeled dataset. In practice, one may resort to standard techniques in the positive-unlabeled (PU) learning literature to estimate this quantity (e.g., \citet{garg2021mixture}). 

\textit{Plug-in classifier:} Having obtained probability estimates
 $\hat{\Pr}_{\rm in}(y|x) = \frac{\exp( \hat{f}_y(x)) }{ \sum_{y' \in [L]} \exp( \hat{f}_{y'}(x)) }$ and $\hat{\eta}_{\rm mix}(x) = \psi^{-1}( \hat{r}(x) )$
 using the logits
$\hat{f}$ and scorer $\hat{r}$ from the first step,
 and then estimates of the OOD conditional distribution $\hat{\eta}_{\rm out}(x)$ using the transformation %in Lemma \ref{lem:wild-noise-correction} 
 in the second step, we can now approximate the Bayes-optimal classifier in Lemma \ref{lem:ood-constrained-bayes}:
\begin{align*}
    \hat{h}(x) &= 
            \begin{cases}
                \perp & \text{if}~
                    \hat{z}( x ) > t_{\rm abs}
                    \\
                \argmax_{y \in [L]}\hat{\Pr}_{\rm in}(y|x) &
                \text{else}
            \end{cases}, \\
    \text{where}&~\hat{z}( x ) \defEq (1 - \hat{\eta}_{\rm out}(x)) \cdot \left(1 - \max_{y \in [L]}\hat{\Pr}_{\rm in}(y|x) \right)  \\
    &
    \hspace{4.7cm} + \hat{\eta}_{\rm out}(x) \cdot c_{\rm ood}.
\end{align*}
The threshold $t_{\rm abs}$ needs to be chosen so that the proportion of abstentions on the test population is at most $B_{\rm abs}$. Equivalently, one can pick $t_{\rm abs}$ using the training sample, and choose it to be the smallest value for which the following inlier-proportion-corrected budget constraint holds:
\begin{align*}
\lefteqn{ 
\textstyle
\frac{1}{1 - \pi_{\rm in}} \cdot \frac{1}{N} \sum_{i=1}^N \1( \hat{z}(x^u_i) > t_{\rm abs} )  }\\
&
\textstyle
+ \frac{1 - 2\pi_{\rm in}}{1 - \pi_{\rm in}} \cdot \frac{1}{N} \sum_{i=1}^N \1( \hat{z}(x_i)  > t_{\rm abs})
< B_{\rm abs}.
\end{align*}

% \if 0
Using the characterization in Lemma \ref{lem:ood-wild-bayes}, one can construct a plug-in estimator for the Bayes classifier from estimates of the conditional distributions $\Pin(y|x)$ and $\eta_{\rm mix}(x)$. The proposed approach would work in two stages: (i) optimize a base loss function similar to \citet{Thulasidasan:2021} on the inlier and unlabeled  samples to obtain estimates of $\Pin(y|x)$ and $\eta_{\rm mix}(x)$; (ii) construct the classifier in Lemma \ref{lem:ood-bayes} by plugging in the obtained estimates.
%
\begin{align*}
    \eta_{\rm out}(x) 
        &= \frac{ \Pr_{\rm out}(x)}{
                \Pr_{\rm in}(x) + 
                \Pr_{\rm out}(x)}\\
    \eta'_{\rm out}(x) 
        &= \frac{ \Pr_{\rm out}(x)}{
                \Pr_{\rm in}(x) + 
                \Pr_{\rm mix}(x)}\\
    \eta_{\rm mix}(x) 
        &= \frac{ \Pr_{\rm mix}(x)}{
                \Pr_{\rm in}(x) + 
                \Pr_{\rm mix}(x)}\\
        &= \frac{\pi_{\rm in} \cdot \Pin(x) + 
                (1 - \pi_{\rm in} ) \cdot \Pout(x)}{
                \Pin(x) + \Pr_{\rm mix}(x)}\\
        % &= Z(x)\cdot \frac{\pi_{\rm in} \cdot \Pin(x) + 
        %         (1 - \pi_{\rm in} ) \cdot \Pout(x)}{
        %         \Pin(x) + \Pr_{\rm out}(x)}\\
        &= \pi_{\rm in} \cdot ( 1 - \eta_{\rm mix}(x) ) + 
                (1 - \pi_{\rm in} ) \cdot \eta'_{\rm out}(x),
\end{align*}
from which we have:
\begin{align*}
    \eta'_{\rm out}(x) &= \frac{1}{1 - \pi_{\rm in}} \cdot ((1 + \pi_{\rm in}) \cdot \eta_{\rm mix}(x) - \pi_{\rm in}).
\end{align*}
Furthermore,
\begin{align*}
    \eta_{\rm out}(x) &= \frac{\eta'_{\rm out}(x) }{\eta'_{\rm out}(x)  + 1 - \eta_{\rm mix}(x)}\\
    &=  \frac{ (1 + \pi_{\rm in}) \cdot \eta_{\rm mix}(x) - \pi_{\rm in} }{2\pi_{\rm in} \cdot \eta_{\rm mix}(x) + 1 - 2\pi_{\rm in}}.
\end{align*}
% \fi


\subsection{Contrasting with \citet{Katz:2022}}
Like us, \citet{Katz:2022} also seek to jointly learn a classifier and an OOD scorer, with  constraints  on the classification and abstention rates, given access to samples from $\Pr_{\rm in}$ and $\Pr_{\rm mix}$. %Specifically, they seek to minimize the proportion of non-abstained OOD samples  subject to constraints on the proportion of abstained inlier examples and the error rate on the inlier examples. 
For a joint classifier $h: \XCal \rightarrow [L] \cup \{\perp\}$, their formulation can be written as:
% \begin{align}
%   \lefteqn{
%   \min_{h}~
%   \Ex_{x \sim \Pr_{\rm out}}\left[ \1\left( h(x) \ne \perp \right) \right] }
%   \label{eq:ks-original}
%   \\
%     \text{s.t.}\hspace{10pt}
%     & \Ex_{x \sim \Pin}\left[ \1\left( h(x) = \perp \right) \right] \leq \alpha
%     \nonumber
%     \\
%     & \Ex_{(x, y) \sim \Pin}\left[ \1\left( h(x) \ne y,\, h(x) \ne \perp \right) \right]  \leq \tau,
%     \nonumber
% \end{align}
\begin{align}
   \lefteqn{
   \min_{h}~
   \Pr_{\rm out}\left( h(x) \ne \perp \right) }
   \label{eq:ks-original}
   \\
    \text{s.t.}\hspace{20pt}
    & \Pin\left( h(x) = \perp \right) \leq \alpha
    \nonumber
    \\
    & \Pin\left( h(x) \ne y,\, h(x) \ne \perp \right)  \leq \tau,
    \nonumber
\end{align}
for given targets $\alpha, \beta \in (0,1)$. 

While $\Pr_{\rm out}$ is not directly available, 
\citeauthor{Katz:2022} provide a simple solution to solving  \eqref{eq:ks-original} using only access to $\Pr_{\rm mix}$ and $\Pr_{\rm in}$. They show that under some mild assumptions,  replacing  $\Pr_{\rm out}$ with $\Pr_{\rm mix}$ in the above problem does not alter the optimal solution. The intuition behind this is that when the first constraint on the inlier abstention rate is satisfied with equality, we have $\Ex_{x \sim \Pr_{\rm mix}}\left[ \1\left( h(x) \ne \perp \right) \right] = \pi_{\rm in} \cdot (1 - \alpha) + (1 - \pi_{\rm in}) \cdot \Ex_{x \sim \Pr_{\rm out}}\left[ \1\left( h(x) \ne \perp \right) \right]$, and minimizing this objective is equivalent to minimizing the OOD objective in \eqref{eq:ks-original}. 

This simple trick of replacing $\Pr_{\rm out}$ with $\Pr_{\rm mix}$ will only work when we have an explicit constraint on the inlier abstention rate, and will not work for the formulation we are interested in \eqref{eqn:budget-constrainted-ood}. This is because in our formulation, we impose a budget on the overall abstention rate (as this is a more intuitive quantity that a practitioner may want to constraint), and do not explicitly control the abstention rate on $\Pr_{\rm in}$. 

In comparison to \citet{Katz:2022}, the plug-in based approach we prescribe is more general, and can be applied to optimize any objective that involves as a weighted combination of the mis-classification error and the abstention rates on the inlier and OOD samples. This includes both the  budget-constrained problem we consider in \eqref{eqn:budget-constrainted-ood}, and the constrained problem of \citeauthor{Katz:2022} in \eqref{eq:ks-original}.

%Furthermore, the authors  propose replacing the non-differentiable indicator functions in  with smooth surrogates, and solving the relaxed optimization problem. 

% Notice that the formulation we propose in \eqref{eqn:budget-constrainted-ood} is equivalent to \eqref{eq:ks-original} for a particular choice of cost penalty $c_{\rm ood}$. However, 

% The formulation we propose in \eqref{eqn:budget-constrainted-ood} is similar in flavor, but requires the practitioner to specify a budget on the overall abstention rate (not just that on the inlier samples), and the trade-off between the classification error and OOD detection rate is specified through a cost penalty $c_{\rm ood}$ rather than a constraint on the classification error. 

% Importantly, our solution approach is very different. Instead of replacing the objective with a noisy approximation and relaxing it further with smooth surrogates, we directly estimate the conditional statistics involved by using tools from the PU learning literature, and construct the optimal classifier from the obtained estimates. Our approach is more flexible, in that, it allows for the use of any loss function that can estimate the inlier class probabilities $\Pr_{\rm in}(y|x)$ and the density ration $\frac{\Pr_{\rm in}(x)}{\Pr_{\rm mix}(x)}$, and the final classifier uses simple a post-hoc transformation on the estimated quantities.

% {
% \color{blue}
% TODO: Is there a compelling way to differentiate ourselves from \citet{Katz:2022}?
% }

==> icml2023/relation.tex <==
{Given the failure of the MSP baseline for general OOD detection, one may ask: 
is there some other method that may fare better at jointly handling the L2R and OOD detection problems?}
%
% To better understand the connection between L2R and OOD detection,
To answer this question,
it is useful to spell out a joint classification risk.
{We do so for a general setting, where the OOD samples are not necessarily from an unseen class, but can come from an arbitrary distribution $\Pr_{\rm out}$.}
% \todoakm{Clarify that we are no longer in the open-set setting?}

%
\subsection{OOD-aware misclassification error}

{
Recall that OOD detection concerns learning a detector $r \colon \XCal \to \{ 0, 1 \}$.
For practical deployment in classification settings,
it is natural to use this detector to abstain from making a prediction on
% in practice, such a detector is likely to be coupled with a standard classifier, so that the latter can abstain on 
samples deemed to be OOD~\citep{Bitterwolf:2022,Xia:2022}.
% In such settings, a natural goal is to maximise classification accuracy on samples deemed inliers, while allowing for abstention on OOD samples.
% Of course,
% % In addition to abstention on OOD samples, 
% it is natural to 
As with the L2R problem, one may
additionally allow for abstention on in-distribution (but ``hard'') samples.
Intuitively, these two abstentions have different costs:
e.g., there may be monetary cost for abstaining on an inlier sample,
but a cost to reputation due to an embarrassingly wrong prediction for \emph{failing} to abstain on OOD samples.}

To formalise this,
we assume that a classifier is allowed the additional option of predicting that a sample is OOD, denoted by  $\abstain$.
% \todoakm{Should we just use $\perp$ here?
% Hari: yep, agreed! 
% }
Furthermore, there is a cost $\costin \in \Real$ associated with classifying an inlier example as OOD, and a cost $\costout \in \Real$ associated with classifying an OOD example as inlier.
Our goal is
to then learn an \emph{abstention-augmented} classifier $\bar{h} \colon \XCal \to \YCal \cup \{ \abstain \}$ to minimise the 
following \emph{joint} objective:
% \emph{joint OOD-aware} misclassification error:
% \todoakm{We are here using $h$ as opposed to $\bar{h}$, or $h$ and $r$}
\begin{align}
    \label{eqn:ood}
    R_{\rm joint}( \bar{h} ) &\defEq 
    % \Pr_{\rm in}( y \neq h( x ) ) \,+\, \\
    \Pr_{\rm in}( y \neq \bar{h}( x ), \bar{h}( x ) \neq \abstain ) + 
    % \\
    % \nonumber
    % &
    \costin \cdot \Pr_{\rm in}( \bar{h}( x ) = \abstain ) + \costout \cdot \Pr_{\rm out}( \bar{h}( x ) \neq \abstain ).
\end{align}
This simply combines the usual misclassification error of $h$ with explicit penalties for OOD detection errors.
{Similar objectives have been implicitly considered in~\citet{Bitterwolf:2022,Katz:2022}.}
% \todoakm{Is any of this implicit in Bitterwolf et al.? Hari: In Bitterwolf, when they define the de-coupled CE loss in Page 6, they allow for asymmetric weighting. Also, Katz-Samuels explicitly define the TPR and FPR for OOD detection and impose constraints on them. Later when they formulate an augmented Lagrangian for their constraints, it implicit that they impose costs on the OOD detection errors. They do not derive the Bayes-optimal classifier. Should we add a remark here noting this  similarity to these papers?}

%
% Note that 
% one can equally write~\eqref{eqn:ood} as 
% \begin{align*}
%     R_{\rm ood}( h ) &= 
%     \Pr_{\rm in}( y \neq h( x ), h( x ) \neq \abstain ) + \\
%     &(\costin + 1) \cdot \Pr_{\rm in}( h( x ) = \abstain ) + \costout \cdot \Pr_{\rm out}( h( x ) \neq \abstain ),
% \end{align*}
% since by definition $\Pr_{\rm in}( y \neq h( x ), h( x ) = \abstain ) = \Pr_{\rm in}( h( x ) = \abstain )$.
% Thus,

%
\textbf{Remark}.
Notice that
interpreting the prediction $\abstain$ as abstention,
the first two terms are precisely the standard learning to reject risk applied to the inlier distribution $\Pr_{\rm in}$. In other words, when we set $\costout$ to 0, the above joint risk reduces to that for L2R, i.e., to the {abstention-aware risk} in \eqref{eqn:abstention-aware-risk}.


%
\subsection{OOD detection as sample-dependent Chow's rule}

Below, we derive the Bayes-optimal classifier for~\eqref{eqn:ood}. 
% the joint OOD-aware misclassification error. % in \eqref{eqn:ood}.

%
\begin{lemma}[Bayes-optimal classifier for~\eqref{eqn:ood}]
\label{lem:ood-bayes}
%Let $\eta_{\rm out}( x ) = \frac{ 1 }{ 1 + \frac{ \Pr_{\rm in}(x) }{ \Pr_{\rm out}(x) }}$.
The minimizer of \eqref{eqn:ood} predicts for any $x \in \cX$ with $\Pr_{\rm in}( x ) > 0$:
\begin{align}
    \nonumber
    \bar{h}^*(x) &= 
            \begin{cases}
                \abstain & \text{if}~
                    %z( x ) > 0
                    \displaystyle
                    \max_{y \in [L]}\Pr_{\rm in}(y|x) < t(x)
                    \\
                {\displaystyle
                \underset{y \in [L]}{\argmax}\,\Pr_{\rm in}(y|x)} &
                \text{else,}
            \end{cases}
    \\
    % \text{where}&~z( x ) ~\defEq (1 - \eta_{\rm out}(x)) \cdot \left(1 - \max_{y \in [L]}\Pr_{\rm in}(y|x) - \costin \right)  \\
    % &
    % \hspace{4.5cm} + \eta_{\rm out}(x) \cdot \costout.
%  \end{align*}
% where
% \begin{align}
    t( x ) &\defEq 1 - \costin + \costout \cdot \frac{\Pr_{\rm out}( x )}{\Pr_{\rm in}( x )}.
    \label{eqn:joint-ood-bayes}
\end{align}
For any instance $x$ with $\Pr_{\rm in}( x ) = 0$,  $\bar{h}^*(x) = \abstain$.
\end{lemma}

%
Similar to the Bayes-optimal classifier in \eqref{eqn:chow} for L2R, the 
above also thresholds the inlier conditional-class probability to decide which samples to abstain on.
A key difference however is that we use an \emph{instance-dependent} threshold: the abstention rule uses both 
inlier $\Pr_{\rm in}( y \mid x )$ 
\emph{and} 
the inverse density ratio $\frac{\Pr_{\rm out}( x )}{\Pr_{\rm in}( x )}$ to decide when to abstain. 
% In the special case, 

Observe that when $\costout = 0$ and $\alpha \in [0, 1]$, 
we get the Bayes-optimal classifier for learning to reject in \eqref{eqn:chow}, with a constant threshold $t(x) = 1 - \costin$. %, which abstains only on samples where the inlier conditional-class probability falls below a threshold:
% $$\max_{y \in [L]}\Pr_{\rm in}(y|x) < 1 - \costin.$$
% \todoakm{I wonder if we could have a subsection title that calls out that OOD = Sample-dependent Chow}
{On the other hand, 
if $\beta > \alpha \cdot \frac{\Pr_{\rm in}( x )}{\Pr_{\rm out}( x )}$
for a given $x$, 
we will always abstain.}
% Otherwise, for any given $x$, when $\costout \in \left(0, \alpha \cdot \frac{\Pr_{\rm in}( x )}{\Pr_{\rm out}( x )}\right)$, we get an instance-dependent threshold $t(x) < 1$.
% \todoakm{Not sure if spelling out the range for $\beta$ makes it more confusing. The range is now instance dependent, and we would need to clarify that this applies only when $\Pr_{\rm out}( x ) > 0$.}
% \todoakm{Spell out range of $\beta$}

%
{\textbf{Open-set classification redux}.
{We now revisit the open-set classification problem introduced in Figure~\ref{fig:chow-fail-example-open-set}.
% ~\S\ref{sec:chow-fail-open-set}.
Recall that here, the maximum inlier class-probabilities 
$\max_y \Pr_{\rm in}( y \mid x )$ 
are higher for outlier compared to inlier samples.
Figure~\ref{fig:max_prob_instance_threshold_synthetic} shows the distribution of the sample-dependent thresholds $t( x )$ on $\max_y \Pr_{\rm in}( y \mid x )$,
as contrasted with the constant threshold $1 - \alpha$ applied by vanilla MSP.
% Here, we set $\alpha = 0.5$ and $\beta = 2.0$.
% \todoakm{Fix this, $\alpha = 0$ will be a trivial solution...}
% \todoakm{Edit this as needed}
% \todoakm{Should we mention AUC in the previous section also? Commented it out for the time-being in the interest of space.}
The results are intuitive: 
we place a \emph{higher} threshold on outlier samples, 
so that they are correctly rejected by $\bar{h}^*$ despite having high $\max_y \Pr_{\rm in}( y \mid x )$.
In Appendix~\ref{app:expts-impact-alpha-beta}, we visualise the impact of varying $\alpha, \beta$ on abstentions in this example.}
% as compared to inlier samples.
}
% %%% Hari: we could perhaps move this to the appendix.
% Employing such a sample-dependent threshold has a significant effect on OOD detection performance.
% The AUC-ROC for  OOD detection (of the resulting scorer) improves to {\bf 96\%} compared to {\bf 29\%} when 
% % scoring with the maximum probability.
% using a static threshold.
% %%% 

%
\begin{figure}[!t]
    \centering
    %
    \resizebox{0.6\linewidth}{!}{
        % \includegraphics[scale=0.25]{figs/max_prob_instance_threshold_synthetic.pdf}
        \includegraphics[scale=0.25]{figs/max_prob_instance_threshold_synthetic_v2.pdf}
    }
    \vspace{-5pt}
    \caption{Distribution of instance-dependent maximum softmax probability threshold for the synthetic open-set classification problem in~\S\ref{sec:chow-fail-open-set}, for costs 
    $\alpha = 0.95$ and $\beta = 0.1$.
    % There is significant variation in thresholds for samples, as opposed to the static threshold employed by vanilla MSP (shown in black).
    As is intuitive, 
    we place a \emph{higher} threshold on outlier as compared to inlier samples,
    as opposed to the static threshold employed by vanilla MSP (black).
    }
    \vspace{-5pt}
    \label{fig:max_prob_instance_threshold_synthetic}
\end{figure}

% \todoakm{Maybe have a result on one of the synthetic problems? Hari: agreed, will get to this once I wrap up the expt baselines.}



% \todo[inline]{Can we simplify the bracketed term to be $-\max \Pr_{\rm in} - \costout$?}

% One may augment a regular classifier with an OOD option by
% learning a scorer $f \colon \XCal \to \Real^{L + 1}$, with an additional OOD score $f_{\abstain}( x )$,
% and predicting a sample to be OOD iff $\gamma_{\abstain}( x ) \defEq f_{\abstain}( x ) - \max_{y' \in [ L ]} f_{y'}( x ) > 0.$

% As an alternative to~\eqref{eqn:ood},
% one may also measure the \emph{pairwise ranking} performance of the OOD detector,
% in the form of the \emph{AUC-ROC}:
% \begin{align*}
%     R_{\rm ood}( f ) &\defEq 
%     \Pr_{\rm in}( y \neq \argmax_{y' \in [L]} f_{y'}( x ) ) + \\
%     &\mathbb{E}_{x \sim \Pr_{\rm in}} \mathbb{E}_{x' \sim \Pr_{\rm out}} \indicator{ \gamma_{\abstain}( x ) > \gamma_{\abstain}( x' ) }.
% \end{align*}


%
% \subsection{Discussion: contrasting L2R and OOD detection}

{Recently,~\citet{Xia:2022} also considered the problem of jointly performing OOD detection, and abstaining on hard samples.
However, they 
did not explicate the failure cases of the MSP baseline;
did not explicate the form of the Bayes-optimal solution;
and proposed a heuristic solution.
}

% \hari{Should this section come after the next section on sub-optimality? I ask this because again in the next section we talk about Bayes-optimal classifiers, which assumes an objective different from the one in \eqref{eqn:ood}.}

% \todo[inline]{Agreed, and indeed it could be nice to start off by noting there's a connection between baselines for these problems --- which we dive into --- and to then talk about the formal connection more generally.}

